The complex volume of SL(n,C)-representations of 3-manifolds

For a compact 3-manifold M with arbitrary (possibly empty) boundary, we give a parametrization of the set of conjugacy classes of boundary-unipotent representations of the fundamental group of M into SL(n,C). Our parametrization uses Ptolemy coordinates, which are inspired by coordinates on higher Teichmueller spaces due to Fock and Goncharov. We show that a boundary-unipotent representation determines an element in Neumann's extended Bloch group, and use this to obtain an efficient formula for the Cheeger-Chern-Simons invariant, and in particular for the volume. Computations for the census manifolds show that boundary-unipotent representations are abundant, and numerical comparisons with census volumes, suggest that the volume of a representation is an integral linear combination of volumes of hyperbolic 3-manifolds. This is in agreement with a conjecture of Walter Neumann, stating that the Bloch group is generated by hyperbolic manifolds.

==> draws/SLrepFigures <==
u:=1cm;
pair cuta[];
cuta0:=(0,0);cuta2:=u*dir(0);cuta1:=u*dir(60);cuta3:=cuta1+cuta2;
pair cutb[];
 for i=0 upto 4:
  cutb[i]:=cuta[i]+dir(60)*3u;
 endfor;
pair cutc[];
 for i=0 upto 4:
  cutc[i]:=cuta[i]+dir(0)*3u;
 endfor;
pair cutd[];
for i=0 upto 4:
  cutd[i]:=cutc[i]+dir(60)*3u;
 endfor;

pair a;pair b; pair c; pair d; pair ds;
a:=cuta0;b:=cuta1+dir(60)*5u;c:=cuta2+dir(0)*5u;ds:=cuta3+dir(0)*5*u+dir(60)*5u;d:=ds-(1.4*u,-0.5*u);

path ee[];pair CC;ee1:=a--1/2[b,c];ee2:=b--1/2[a,c];CC:=ee1 intersectionpoint ee2;

input cmarrows;

setup_cmarrows(
  arrow_name     = "twoheadarrow";
  parameter_file = "cmr25.mf";
  macro_name     = "doublearrow");

setup_cmarrows(
  arrow_name     = "shortaxisarrow";
  parameter_file = "cmr25.mf";
  macro_name     = "singlearrow");

setup_cmarrows(
  arrow_name     = "shortaxisarrow";
  parameter_file = "cmr10.mf";
  macro_name     = "smallsinglearrow");


def whitearrow expr p = _apth:=p; _finwhitearr enddef;

  def _finwhitearr text t =
    draw _apth t;
    fill arrowhead _apth  t withcolor white;
    draw arrowhead _apth  t
  enddef;


%example: doublearrow (60pt,10pt)--(95pt,45pt);


beginfig(1);
pickup pencircle scaled 1.5pt;
draw a--c; draw b--c; draw c--d;
draw b--d; draw a--c; draw a--b;
draw a--0.52*d; draw 0.58*d--d;
dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.ulft(btex $1$ etex scaled 1.8,b);
dotlabel.lrt(btex $2$ etex scaled 1.8,c);
dotlabel.urt(btex $3$ etex scaled 1.8,d);
%label.lft(btex $c_{01}$ etex scaled 1.8,1/2[a,b]);
%label.rt(btex $c_{23}$ etex scaled 1.8,1/2[c,d]);
%label.ulft(btex $c_{03}$ etex scaled 1.8,1/2[a,d]);
%label.rt(btex $c_{12}$ etex scaled 1.8,1/2[b,c]+(0.1*u,0));
%label.bot(btex $c_{02}$ etex scaled 1.8,1/2[a,c]);
%label.top(btex $c_{13}$ etex scaled 1.8,1/2[b,d]);

draw 1/2[a,b] withpen pencircle scaled 4bp;
draw 1/2[c,d] withpen pencircle scaled 4bp;
draw 1/2*d withpen pencircle scaled 4bp;
draw 1/2[b,c] withpen pencircle scaled 4bp;
draw 1/2[a,c] withpen pencircle scaled 4bp;
draw 1/2[b,d] withpen pencircle scaled 4bp;

endfig;


beginfig(2);

pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;

dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.ulft(btex $1$ etex scaled 1.8,b);
dotlabel.lrt(btex $2$ etex scaled 1.8,c);
dotlabel.urt(btex $3$ etex scaled 1.8,d);

draw 1/3[a,b] withpen pencircle scaled 4bp;
draw 2/3[a,b] withpen pencircle scaled 4bp;
draw 1/3[a,c] withpen pencircle scaled 4bp;
draw 2/3[a,c] withpen pencircle scaled 4bp;
draw 1/3[a,d] withpen pencircle scaled 4bp;
draw 2/3[a,d] withpen pencircle scaled 4bp;
draw 1/3[b,d] withpen pencircle scaled 4bp;
draw 2/3[b,d] withpen pencircle scaled 4bp;
draw 1/3[b,c] withpen pencircle scaled 4bp;
draw 2/3[b,c] withpen pencircle scaled 4bp;
draw 1/3[c,d] withpen pencircle scaled 4bp;
draw 2/3[c,d] withpen pencircle scaled 4bp;

draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;
draw 1/2[2/3[b,c],2/3[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/3[a,b],2/3[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/3[a,d],1/3[c,d]] withpen pencircle scaled 4bp;

draw 1/3[a,b]--2/3[b,c] dashed evenly;
draw 1/3[a,b]--2/3[b,d] dashed evenly;
draw 1/3[c,b]--1/3[d,b] dashed evenly;

endfig;

beginfig(3);

pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;

dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.ulft(btex $1$ etex scaled 1.8,b);
dotlabel.lrt(btex $2$ etex scaled 1.8,c);
dotlabel.urt(btex $3$ etex scaled 1.8,d);

draw 1/2[a,b] withpen pencircle scaled 4bp;
draw 1/2[a,c] withpen pencircle scaled 4bp;
draw 1/2[a,d] withpen pencircle scaled 4bp;
draw 1/2[b,c] withpen pencircle scaled 4bp;
draw 1/2[b,d] withpen pencircle scaled 4bp;
draw 1/2[c,d] withpen pencircle scaled 4bp;

draw 1/4[a,b] withpen pencircle scaled 4bp;
draw 1/4[a,c] withpen pencircle scaled 4bp;
draw 1/4[a,d] withpen pencircle scaled 4bp;
draw 1/4[b,c] withpen pencircle scaled 4bp;
draw 1/4[b,d] withpen pencircle scaled 4bp;
draw 1/4[c,d] withpen pencircle scaled 4bp;

draw 3/4[a,b] withpen pencircle scaled 4bp;
draw 3/4[a,c] withpen pencircle scaled 4bp;
draw 3/4[a,d] withpen pencircle scaled 4bp;
draw 3/4[b,c] withpen pencircle scaled 4bp;
draw 3/4[b,d] withpen pencircle scaled 4bp;
draw 3/4[c,d] withpen pencircle scaled 4bp;

draw 1/2[1/2[b,c],1/2[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/2[b,c],1/2[c,d]] withpen pencircle scaled 4bp;
draw 1/2[1/2[b,d],1/2[c,d]] withpen pencircle scaled 4bp;

draw 1/2[1/2[a,c],1/2[c,d]] withpen pencircle scaled 4bp;
draw 1/2[1/2[a,d],1/2[c,d]] withpen pencircle scaled 4bp;
draw 1/2[1/2[a,c],1/2[a,d]] withpen pencircle scaled 4bp;

draw 1/2[1/2[a,b],1/2[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/2[a,d],1/2[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/2[a,b],1/2[a,d]] withpen pencircle scaled 4bp;

draw 1/2[1/2[a,b],1/2[b,c]] withpen pencircle scaled 4bp;
draw 1/2[1/2[a,c],1/2[b,c]] withpen pencircle scaled 4bp;
draw 1/2[1/2[a,b],1/2[a,c]] withpen pencircle scaled 4bp;

draw 1/2[(1/2[1/2[a,b],1/2[a,d]]),(1/2[1/2[b,c],1/2[c,d]])] withpen pencircle scaled 4bp;

draw 1/2[1/2[a,b],1/2[a,c]]--3/4[b,c] dashed evenly;
draw 3/4[b,c]--1/2[1/2[b,d],1/2[c,d]] dashed evenly;
draw 1/2[1/2[a,b],1/2[a,c]]--1/2[1/2[b,d],1/2[c,d]] dashed evenly;
draw 1/2[1/2[a,b],1/2[a,c]]--1/4[b,c] dashed evenly;
draw 1/4[b,c]--1/2[1/2[b,d],1/2[c,d]] dashed evenly;

endfig;

beginfig(4);
pickup pencircle scaled 1.5pt;

draw a--b--c--a;

label.urt(btex $$ etex scaled 1.8,d);

draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;

draw 1/3[a,b] withpen pencircle scaled 4bp;
draw 2/3[a,b] withpen pencircle scaled 4bp;
draw 1/3[a,c] withpen pencircle scaled 4bp;
draw 2/3[a,c] withpen pencircle scaled 4bp;
draw 1/3[b,c] withpen pencircle scaled 4bp;
draw 2/3[b,c] withpen pencircle scaled 4bp;

draw 1/3[a,b]--1/3[c,b] dashed evenly;
draw 1/3[a,c]--1/3[b,c] dashed evenly;
draw 1/3[b,a]--1/3[c,a] dashed evenly;

dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.top(btex $1$ etex scaled 1.8,b);
dotlabel.lrt(btex $2$ etex scaled 1.8,c);

endfig;


beginfig(5);
pickup pencircle scaled 1.5pt;

draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;


draw 1/3[a,b] withpen pencircle scaled 4bp;
draw 2/3[a,b] withpen pencircle scaled 4bp;
draw 1/3[a,c] withpen pencircle scaled 4bp;
draw 2/3[a,c] withpen pencircle scaled 4bp;
draw 1/3[a,d] withpen pencircle scaled 4bp;
draw 2/3[a,d] withpen pencircle scaled 4bp;
draw 1/3[b,d] withpen pencircle scaled 4bp;
draw 2/3[b,d] withpen pencircle scaled 4bp;
draw 1/3[b,c] withpen pencircle scaled 4bp;
draw 2/3[b,c] withpen pencircle scaled 4bp;
draw 1/3[c,d] withpen pencircle scaled 4bp;
draw 2/3[c,d] withpen pencircle scaled 4bp;

draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;
draw 1/2[2/3[b,c],2/3[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/3[a,b],2/3[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/3[a,d],1/3[c,d]] withpen pencircle scaled 4bp;

draw 1/3[b,a]--1/3[c,a] dashed evenly;
draw 1/3[c,a]--1/3[d,a] dashed evenly;
draw 1/3[d,a]--1/3[b,a] dashed evenly;

dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.ulft(btex $1$ etex scaled 1.8,b);
dotlabel.lrt(btex $2$ etex scaled 1.8,c);
dotlabel.urt(btex $3$ etex scaled 1.8,d);

endfig;

beginfig(6);
pair a[]; pair e[];

pickup pencircle scaled 0.4pt;

a6:=(0,0);a1:=(0.4,1.4)*u;a2:=(1.4,1.4)*u;
a3:=(0,1)*u;a4:=(1,1)*u;a5:=(1.4,0.5)*u;a7:=(1,0)*u;
e1:=1/2[a1,a2];e2:=1/2[a3,a1];e3:=1/2[a4,a2];e4:=1/2[a3,a4];e5:=1/2[a3,a6];
e6:=1/2[a4,a7];e7:=1/2[a2,a5];e8:=1/2[a6,a7];e9:=1/2[a5,a7];

draw a3--a4--a7--a6--a3--a1--a2--a5--a7--a4--a2;

draw e5--e6--e7;draw e8--e4--e1;draw e2--e3--e9;

draw a6--a4--a1;draw a7--a3--a2;draw a2--a7;draw a5--a4;

endfig;

beginfig(7);

pair a[];
a1:=(0,0);a2:=(0,1)*u;a3:=(1,0)*u;;

whitearrow a1--a2 withpen pencircle scaled 1bp;
doublearrow a1--a3 withpen pencircle scaled 1bp;
singlearrow  a2--a3 withpen pencircle scaled 1bp;

endfig;

beginfig(8);%truncated simplex with labelings.

pickup pencircle scaled 1pt;

draw cuta0--cuta1 dashed evenly scaled 1;
draw cuta0--cuta2 dashed evenly scaled 1;
smallsinglearrow  cuta1--1/2[cuta1,cuta3] withpen pencircle scaled 1bp;draw 1/2[cuta1,cuta3]--cuta3;
smallsinglearrow  cuta2--1/2[cuta3,cuta2] withpen pencircle scaled 1bp;draw 1/2[cuta3,cuta2]--cuta3;
smallsinglearrow  cuta1--1/2[cuta2,cuta1] withpen pencircle scaled 1bp;draw 1/2[cuta2,cuta1]--cuta2;
draw cuta0--0.4*cuta3 dashed evenly scaled 1;
draw 0.6*cuta3--cuta3 dashed evenly scaled 1;

dotlabel.llft(btex $0$ etex scaled 1.3,cuta0);
dotlabel.ulft(btex $1$ etex scaled 1.3,cutb1);
dotlabel.lrt(btex $2$ etex scaled 1.3,cutc2);
dotlabel.urt(btex $3$ etex scaled 1.3,cutd3);
dotlabel.urt(btex $$ etex,cuta2);
dotlabel.rt(btex $$ etex,cuta3);
dotlabel.lft(btex $$ etex,cuta1);
dotlabel.lft(btex $$ etex,cutb0);
dotlabel.rt(btex $$ etex,cutb2);
dotlabel.top(btex $$ etex,cutb3);
dotlabel.bot(btex $$ etex,cutc0);
dotlabel.lft(btex $$ etex,cutc1);
dotlabel.rt(btex $$ etex,cutc3);
dotlabel.lft(btex $$ etex,cutd0);
dotlabel.top(btex $$ etex,cutd1);
dotlabel.rt(btex $$ etex,cutd2);

draw cutb0--cutb1 dashed evenly scaled 1;
draw cutb1--cutb3 dashed evenly scaled 1;
smallsinglearrow  cutb2--1/2[cutb2,cutb3] withpen pencircle scaled 1pt;draw 1/2[cutb2,cutb3]--cutb3; 
smallsinglearrow  cutb0--1/2[cutb0,cutb2] withpen pencircle scaled 1pt;draw 1/2[cutb0,cutb2]--cutb2;
draw cutb1--cutb2 dashed evenly scaled 1;
smallsinglearrow  cutb0--3/4[cutb0,(cutb0+0.4*cuta3)] withpen pencircle scaled 1pt;
draw 3/4[cutb0,(cutb0+0.4*cuta3)]--(cutb0+0.4*cuta3);
draw (cutb0+0.6*cuta3)--cutb3;

smallsinglearrow  cutc0--1/2[cutc1,cutc0] withpen pencircle scaled 1pt;draw 1/2[cutc1,cutc0]--cutc1;
smallsinglearrow  cutc1--1/2[cutc1,cutc3] withpen pencircle scaled 1pt;draw 1/2[cutc1,cutc3]--cutc3;
draw cutc2--cutc3 dashed evenly scaled 1;
draw cutc0--cutc2 dashed evenly scaled 1;
draw cutc1--cutc2 dashed evenly scaled 1;
draw cutc0--(cutc0+0.4*cuta3);
smallsinglearrow  (cutc0+0.6*cuta3)--1/2[(cutc0+0.6*cuta3),cutc3] withpen pencircle scaled 1.2pt;
draw 1/2[(cutc0+0.6*cuta3),cutc3]--cutc3;

smallsinglearrow  cutd0--1/2[cutd0,cutd1] withpen pencircle scaled 1pt;draw 1/2[cutd0,cutd1]--cutd1; 
draw cutd1--cutd3 dashed evenly scaled 1;
draw cutd2--cutd3 dashed evenly scaled 1;
smallsinglearrow  cutd0--1/2[cutd2,cutd0] withpen pencircle scaled 1pt;draw 1/2[cutd2,cutd0]--cutd2;
smallsinglearrow  cutd1--2/3[cutd1,cutd2] withpen pencircle scaled 1pt;draw 2/3[cutd1,cutd2]--cutd2;
draw cutd0--(cutd0+0.4*cuta3) dashed evenly scaled 1;
draw (cutd0+0.6*cuta3)--cutd3 dashed evenly scaled 1;
smallsinglearrow  cuta3--2/3[cuta3,0.4*cutd3] withpen pencircle scaled 1pt;draw 2/3[cuta3,0.4*cutd3]--0.4*cutd3;
draw (0.6*cutd3)--cutd0;

smallsinglearrow  cutb2--1/2[cutb2,cutc1] withpen pencircle scaled 1pt;draw 1/2[cutb2,cutc1]--cutc1;
smallsinglearrow  cuta1--1/2[cuta1,cutb0] withpen pencircle scaled 1pt;draw 1/2[cuta1,cutb0]--cutb0;
smallsinglearrow  cutc3--1/2[cutd2,cutc3] withpen pencircle scaled 1pt;draw 1/2[cutd2,cutc3]--cutd2;
smallsinglearrow  cutb3--1/2[cutd1,cutb3] withpen pencircle scaled 1pt;draw 1/2[cutd1,cutb3]--cutd1;
smallsinglearrow  cuta2--1/2[cutc0,cuta2] withpen pencircle scaled 1pt;draw 1/2[cutc0,cuta2]--cutc0;


label.bot(btex $q_{02}$ etex,1/2[cuta2,cutc0]);
label.lft(btex $q_{01}$ etex,1/2[cutb0,cuta1]);
label.rt(btex $q_{12}$ etex,1/2[cutb2,cutc1]);
label.rt(btex $q_{23}$ etex,1/2[cutc3,cutd2]);
label.top(btex $q_{13}$ etex,1/2[cutb3,cutd1]);
label.rt(btex $q_{03}$ etex,2/3[cuta3,0.4*cutd3]-u*(0,0.08));

label.lft(btex $\alpha^0_{12}$ etex,2/3[cuta0,cuta1]-(0.08,0)*u);
label.top(btex $\alpha^0_{13}$ etex,1/2[cuta3,cuta1]);
label.rt(btex $\alpha^0_{23}$ etex,1/2[cuta3,cuta2]);

label.bot(btex $\alpha^1_{02}$ etex,1/2[cutb0,cutb2]);
label.rt(btex $\alpha^1_{23}$ etex,1/2[cutb2,cutb3]);
label.lft(btex $\alpha^1_{03}$ etex,1/2[cutb0,cutb1]-(0.08,0)*u);

label.lft(btex $\alpha^2_{01}$ etex,1/2[cutc0,cutc1]);
label.top(btex $\alpha^2_{13}$ etex,1/2[cutc3,cutc1]);
label.rt(btex $\alpha^2_{03}$ etex,5/8[cutc2,cutc3]);

label.lft(btex $\alpha^3_{01}$ etex,1/2[cutd0,cutd1]);
label.bot(btex $\alpha^3_{02}$ etex,1/2[cutd2,cutd0]-u*(0.1,0));
label.rt(btex $\alpha^3_{12}$ etex,1/3[cutd2,cutd3]);

endfig;

beginfig(9);
numeric n;n:=7;

pickup pencircle scaled 1pt;

label.llft(btex $i$ etex scaled 1.2,a);
label.top(btex $j$ etex scaled 1.2,b);
label.lrt(btex $k$ etex scaled 1.2,c);

pair p[];path l[];

p1:=(n-1)/n*b;p2:=(n-2)/n*b;p3:=(n-3)/n*b;
p4:=p1+1/n*c;p5:=p2+1/n*c;p6:=p3+1/n*c;

p7:=CC-(0.3,0.3)*u;p8:=p7+1/n*b;p9:=p7+1/n*c;p10:=p9+1/n*b;

p11:=1/n*b;p12:=1/n*c;p13:=p12+1/n*b;
p14:=(n-1)/n*c;p15:=(n-2)/n*c;p16:=p14+1/n*b;p17:=p15+1/n*b;

p18:=p5+1/n*c;p19:=p6+1/n*c;

l1:=p1--p4;l2:=p2--p18;l3:=p3--p19+(0.4,0)*u;
l4:=p8-(0.4,0)*u--p10+(0.4,0)*u;l5:=p7-(0.4,0)*u--p9+(0.4,0)*u;
l6:=p4--p6+dir(-120)*0.4u;l7:=p18--p19+dir(-120)*0.4u;
l8:=p8+dir(60)*0.4u--p7+dir(-120)*0.4u;l9:=p10+dir(60)*0.4u--p9+dir(-120)*0.4u;

l10:=p11--p13+(0.4,0)*u;l11:=p17-(0.4,0)*u--p16;
l12:=p13+dir(60)*0.4u--p12;l13:=p17+dir(60)*0.4u--p15;l14:=p16--p14;


pickup pencircle scaled 1.5pt;

%draw CC withpen pencircle scaled 2.5bp;

%p11:=((p1 shifted -CC) rotated 120) shifted CC;


for i=1 upto 19:
  draw p[i] withpen pencircle scaled 2.5bp;
endfor;

label.ulft(btex $(1,1)$ etex scaled 0.9,p5+(0.20,0.13)*u);
label.ulft(btex $(1,n-1)$ etex scaled 0.9,p12+(0.78,0.13)*u);
label.ulft(btex $(1,2)$ etex scaled 0.9,p6+(0.20,0.13)*u);
label.ulft(btex $(2,1)$ etex scaled 0.9,p19+(0.20,0.13)*u);
label.ulft(btex $(r,s)$ etex scaled 0.9,p9+(0.20,0.13)*u);
label.ulft(btex $(n-1,1)$ etex scaled 0.9,p14+(0.6,0.13)*u);

draw a--b--c--a;

for i=1 upto 11:
  draw l[i] dashed evenly scaled 1;
endfor;

draw subpath(0,0.45) of l12 dashed evenly scaled 1;draw subpath(0.85,1) of l12 dashed evenly scaled 1;
draw subpath(0,0.45) of l13 dashed evenly scaled 1;draw subpath(0.85,1) of l13 dashed evenly scaled 1;
draw subpath(0,0.22) of l14 dashed evenly scaled 1;draw subpath(0.8,1) of l14 dashed evenly scaled 1;

dotlabel.lrt(btex $b$ etex scaled 1,p7);
dotlabel.ulft(btex $c$ etex scaled 1,p8);
dotlabel.lrt(btex $d$ etex scaled 1,p9);
dotlabel.ulft(btex $a$ etex scaled 1,p10);

endfig;

beginfig(10);
label.llft(btex $i$ etex scaled 1.2,a);
label.top(btex $j$ etex scaled 1.2,b);
label.lrt(btex $k$ etex scaled 1.2,c);

pickup pencircle scaled 1.5pt;
draw a--b--c--a;
pair p[];path l[];

p1:=(n-1)/n*b;p2:=(n-2)/n*b;p3:=(n-3)/n*b;
p4:=p1+1/n*c;p5:=p2+1/n*c;p6:=p3+1/n*c;

p7:=CC-(0.3,0.3)*u;p8:=p7+1/n*b;p9:=p7+1/n*c;p10:=p9+1/n*b;

p11:=1/n*b;p12:=1/n*c;p13:=p12+1/n*b;
p14:=(n-1)/n*c;p15:=(n-2)/n*c;p16:=p14+1/n*b;p17:=p15+1/n*b;

p18:=p5+1/n*c;p19:=p6+1/n*c;

l1:=p1--p4;l2:=p2--p18;l3:=p3--p19+(0.4,0)*u;
l4:=p8-(0.4,0)*u--p10+(0.4,0)*u;l5:=p7-(0.4,0)*u--p9+(0.4,0)*u;
l6:=p4--p6+dir(-120)*0.4u;l7:=p18--p19+dir(-120)*0.4u;
l8:=p8+dir(60)*0.4u--p7+dir(-120)*0.4u;l9:=p10+dir(60)*0.4u--p9+dir(-120)*0.4u;

l10:=p11--p13+(0.4,0)*u;l11:=p17-(0.4,0)*u--p16;
l12:=p13+dir(60)*0.4u--p12;l13:=p17+dir(60)*0.4u--p15;l14:=p16--p14;

pair q[];path m[];

for i=1 upto 19:
  q[i]:=p[i] rotatedaround(CC,240) reflectedabout(b,1/2[a,c]);
  draw q[i] withpen pencircle scaled 2.5bp;
endfor;

for i=1 upto 14:
  m[i]:=l[i]:=l[i] rotatedaround(CC,240) reflectedabout(b,1/2[a,c]);
endfor;

for i=1 upto 9:
  draw m[i] dashed evenly scaled 1;
endfor;

draw subpath(0.2,1) of m13 dashed evenly scaled 1;
draw subpath(0,0.22) of m10 dashed evenly scaled 1;draw subpath(0.8,1) of m10 dashed evenly scaled 1;
draw subpath(0,0.22) of m12 dashed evenly scaled 1;draw subpath(0.8,1) of m12 dashed evenly scaled 1;
draw subpath(0,0.4) of m11 dashed evenly scaled 1;draw subpath(0.8,1) of m11 dashed evenly scaled 1;
draw subpath(0,0.22) of m14 dashed evenly scaled 1;draw subpath(0.8,1) of m14 dashed evenly scaled 1;

label.lft(btex $(1,1)$ etex scaled 0.9,q5+(0.01,0)*u);
label.top(btex $(1,n-1)$ etex scaled 0.9,q13);
label.lft(btex $(1,2)$ etex scaled 0.9,q6+(0.02,0)*u);
label.lft(btex $(2,1)$ etex scaled 0.9,q19+(0.02,0)*u);
label.lft(btex $(r,s)$ etex scaled 0.9,q9+(0.01,0)*u);
label.lft(btex $(n-1,1)$ etex scaled 0.9,q14+(0.26,-0.4)*u);

dotlabel.lft(btex $b$ etex scaled 1,q7);
dotlabel.lft(btex $c$ etex scaled 1,q8);
dotlabel.rt(btex $d$ etex scaled 1,q9);
dotlabel.rt(btex $a$ etex scaled 1,q10);


endfig;

beginfig(11);
label.llft(btex $i$ etex scaled 1.2,a);
label.top(btex $j$ etex scaled 1.2,b);
label.lrt(btex $k$ etex scaled 1.2,c);;

pickup pencircle scaled 1.5pt;
draw a--b--c--a;
pair p[];path l[];

p1:=(n-1)/n*b;p2:=(n-2)/n*b;p3:=(n-3)/n*b;
p4:=p1+1/n*c;p5:=p2+1/n*c;p6:=p3+1/n*c;

p7:=CC-(0.3,0.3)*u;p8:=p7+1/n*b;p9:=p7+1/n*c;p10:=p9+1/n*b;

p11:=1/n*b;p12:=1/n*c;p13:=p12+1/n*b;
p14:=(n-1)/n*c;p15:=(n-2)/n*c;p16:=p14+1/n*b;p17:=p15+1/n*b;

p18:=p5+1/n*c;p19:=p6+1/n*c;

l1:=p1--p4;l2:=p2--p18;l3:=p3--p19+(0.4,0)*u;
l4:=p8-(0.4,0)*u--p10+(0.4,0)*u;l5:=p7-(0.4,0)*u--p9+(0.4,0)*u;
l6:=p4--p6+dir(-120)*0.4u;l7:=p18--p19+dir(-120)*0.4u;
l8:=p8+dir(60)*0.4u--p7+dir(-120)*0.4u;l9:=p10+dir(60)*0.4u--p9+dir(-120)*0.4u;

l10:=p11--p13+(0.4,0)*u;l11:=p17-(0.4,0)*u--p16;
l12:=p13+dir(60)*0.4u--p12;l13:=p17+dir(60)*0.4u--p15;l14:=p16--p14;

pair q[];path m[];

for i=1 upto 19:
  q[i]:=p[i] rotatedaround(CC,120);
  draw q[i] withpen pencircle scaled 2.5bp;
endfor;

for i=1 upto 14:
  m[i]:=l[i]:=l[i] rotatedaround(CC,120);
endfor;

for i=1 upto 9:
  draw m[i] dashed evenly scaled 1;
endfor;

draw m13 dashed evenly scaled 1;
draw m14 dashed evenly scaled 1;
draw m12 dashed evenly scaled 1;
draw subpath(0,0.22) of m10 dashed evenly scaled 1;draw subpath(0.6,1) of m10 dashed evenly scaled 1;
draw subpath(0,0.22) of m11 dashed evenly scaled 1;draw subpath(0.8,1) of m11 dashed evenly scaled 1;

label.llft(btex $(1,1)$ etex scaled 0.9,q5+(0.19,-0.14)*u);
label.llft(btex $(1,n-1)$ etex scaled 0.9,q12+(0.16,-0.14)*u);
label.llft(btex $(1,2)$ etex scaled 0.9,q6+(0.19,-0.14)*u);
label.llft(btex $(2,1)$ etex scaled 0.9,q19+(0.19,-0.14)*u);
label.llft(btex $(r,s)$ etex scaled 0.9,q9+(0.17,-0.14)*u);
label.top(btex $(n-1,1)$ etex scaled 0.9,q17);

dotlabel.llft(btex $b$ etex scaled 1,q7);
dotlabel.llft(btex $c$ etex scaled 1,q8);
dotlabel.urt(btex $d$ etex scaled 1,q9);
dotlabel.urt(btex $a$ etex scaled 1,q10);

endfig;

beginfig(12);

pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;

dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.ulft(btex $3$ etex scaled 1.8,b);
dotlabel.lrt(btex $1$ etex scaled 1.8,c);
dotlabel.urt(btex $2$ etex scaled 1.8,d);

draw 1/3[a,b] withpen pencircle scaled 4bp;
draw 2/3[a,b] withpen pencircle scaled 4bp;
draw 1/3[a,c] withpen pencircle scaled 4bp;
draw 2/3[a,c] withpen pencircle scaled 4bp;
draw 1/3[a,d] withpen pencircle scaled 4bp;
draw 2/3[a,d] withpen pencircle scaled 4bp;
draw 1/3[b,d] withpen pencircle scaled 4bp;
draw 2/3[b,d] withpen pencircle scaled 4bp;
draw 1/3[b,c] withpen pencircle scaled 4bp;
draw 2/3[b,c] withpen pencircle scaled 4bp;
draw 1/3[c,d] withpen pencircle scaled 4bp;
draw 2/3[c,d] withpen pencircle scaled 4bp;

draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;
draw 1/2[2/3[b,c],2/3[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/3[a,b],2/3[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/3[a,d],1/3[c,d]] withpen pencircle scaled 4bp;

ahlength:=10;
singlearrow a--1/2[a,b];singlearrow c--1/2[c,b];
doublearrow a--1/2[a,c];doublearrow a--7/24[a,d];
whitearrow c--1/2[c,d];whitearrow d--1/2[b,d];

label.ulft(btex $a_0$ etex scaled 1.5,1/3[a,b]);
label.ulft(btex $a_1$ etex scaled 1.5,2/3[a,b]);
label.bot(btex $b_0$ etex scaled 1.5,1/3[a,c]);
label.bot(btex $b_1$ etex scaled 1.5,2/3[a,c]);
label.ulft(btex $b_0$ etex scaled 1.5,1/3[a,d]);
label.ulft(btex $b_1$ etex scaled 1.5,2/3[a,d]);
label.urt(btex $a_1$ etex scaled 1.5,1/3[b,c]);
label.urt(btex $a_0$ etex scaled 1.5,2/3[b,c]);
label.top(btex $c_1$ etex scaled 1.5,1/3[b,d]);
label.top(btex $c_0$ etex scaled 1.5,2/3[b,d]);
label.urt(btex $c_0$ etex scaled 1.5,1/3[c,d]+(0.1,0)*u);
label.urt(btex $c_1$ etex scaled 1.5,2/3[c,d]+(0.1,0)*u);
label.urt(btex $x_2$ etex scaled 1.5,1/2[1/3[a,b],1/3[c,b]]);
label.urt(btex $x_0$ etex scaled 1.5,1/2[1/3[c,b],1/3[d,b]]);
label.ulft(btex $x_1$ etex scaled 1.5,1/2[1/3[a,b],1/3[d,b]]);
label.ulft(btex $x_3$ etex scaled 1.5,1/2[1/3[a,d],1/3[c,d]]);

endfig;

beginfig(13);

pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;

dotlabel.llft(btex $1$ etex scaled 1.8,a);
dotlabel.ulft(btex $3$ etex scaled 1.8,b);
dotlabel.lrt(btex $2$ etex scaled 1.8,c);
dotlabel.urt(btex $0$ etex scaled 1.8,d);

draw 1/3[a,b] withpen pencircle scaled 4bp;
draw 2/3[a,b] withpen pencircle scaled 4bp;
draw 1/3[a,c] withpen pencircle scaled 4bp;
draw 2/3[a,c] withpen pencircle scaled 4bp;
draw 1/3[a,d] withpen pencircle scaled 4bp;
draw 2/3[a,d] withpen pencircle scaled 4bp;
draw 1/3[b,d] withpen pencircle scaled 4bp;
draw 2/3[b,d] withpen pencircle scaled 4bp;
draw 1/3[b,c] withpen pencircle scaled 4bp;
draw 2/3[b,c] withpen pencircle scaled 4bp;
draw 1/3[c,d] withpen pencircle scaled 4bp;
draw 2/3[c,d] withpen pencircle scaled 4bp;

draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;
draw 1/2[2/3[b,c],2/3[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/3[a,b],2/3[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/3[a,d],1/3[c,d]] withpen pencircle scaled 4bp;

singlearrow d--1/2[b,d];singlearrow 0.52*d--7/24[a,d];
doublearrow a--1/2[a,c];doublearrow a--1/2[a,b];
whitearrow c--1/2[c,b];whitearrow d--1/2[c,d];


label.ulft(btex $b_0$ etex scaled 1.5,1/3[a,b]);
label.ulft(btex $b_1$ etex scaled 1.5,2/3[a,b]);
label.bot(btex $b_0$ etex scaled 1.5,1/3[a,c]);
label.bot(btex $b_1$ etex scaled 1.5,2/3[a,c]);
label.ulft(btex $a_1$ etex scaled 1.5,1/3[a,d]);
label.ulft(btex $a_0$ etex scaled 1.5,2/3[a,d]);
label.urt(btex $c_1$ etex scaled 1.5,1/3[b,c]);
label.urt(btex $c_0$ etex scaled 1.5,2/3[b,c]);
label.top(btex $a_1$ etex scaled 1.5,1/3[b,d]);
label.top(btex $a_0$ etex scaled 1.5,2/3[b,d]);
label.urt(btex $c_1$ etex scaled 1.5,1/3[c,d]+(0.1,0)*u);
label.urt(btex $c_0$ etex scaled 1.5,2/3[c,d]+(0.1,0)*u);
label.urt(btex $x_3$ etex scaled 1.5,1/2[1/3[a,b],1/3[c,b]]);
label.urt(btex $x_0$ etex scaled 1.5,1/2[1/3[c,b],1/3[d,b]]);
label.ulft(btex $y_2$ etex scaled 1.5,1/2[1/3[a,b],1/3[d,b]]);
label.ulft(btex $y_3$ etex scaled 1.5,1/2[1/3[a,d],1/3[c,d]]);

endfig;

beginfig(14);

pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;

dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.ulft(btex $1$ etex scaled 1.8,b);
dotlabel.lrt(btex $2$ etex scaled 1.8,c);
dotlabel.urt(btex $3$ etex scaled 1.8,d);

draw 1/3[a,b] withpen pencircle scaled 4bp;
draw 2/3[a,b] withpen pencircle scaled 4bp;
draw 1/3[a,c] withpen pencircle scaled 4bp;
draw 2/3[a,c] withpen pencircle scaled 4bp;
draw 1/3[a,d] withpen pencircle scaled 4bp;
draw 2/3[a,d] withpen pencircle scaled 4bp;
draw 1/3[b,d] withpen pencircle scaled 4bp;
draw 2/3[b,d] withpen pencircle scaled 4bp;
draw 1/3[b,c] withpen pencircle scaled 4bp;
draw 2/3[b,c] withpen pencircle scaled 4bp;
draw 1/3[c,d] withpen pencircle scaled 4bp;
draw 2/3[c,d] withpen pencircle scaled 4bp;

draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;
draw 1/2[2/3[b,c],2/3[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/3[a,b],2/3[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/3[a,d],1/3[c,d]] withpen pencircle scaled 4bp;

singlearrow a--1/2[a,b];singlearrow a--7/24[a,d];
doublearrow a--1/2[a,c];doublearrow d--1/2[b,d];
whitearrow c--1/2[c,b];singlearrow c--1/2[c,d];


label.ulft(btex $a_0$ etex scaled 1.5,1/3[a,b]);
label.ulft(btex $a_1$ etex scaled 1.5,2/3[a,b]);
label.bot(btex $b_0$ etex scaled 1.5,1/3[a,c]);
label.bot(btex $b_1$ etex scaled 1.5,2/3[a,c]);
label.ulft(btex $a_0$ etex scaled 1.5,1/3[a,d]);
label.ulft(btex $a_1$ etex scaled 1.5,2/3[a,d]);
label.urt(btex $c_1$ etex scaled 1.5,1/3[b,c]);
label.urt(btex $c_0$ etex scaled 1.5,2/3[b,c]);
label.top(btex $b_1$ etex scaled 1.5,1/3[b,d]);
label.top(btex $b_0$ etex scaled 1.5,2/3[b,d]);
label.urt(btex $a_0$ etex scaled 1.5,1/3[c,d]+(0.1,0)*u);
label.urt(btex $a_1$ etex scaled 1.5,2/3[c,d]+(0.1,0)*u);
label.urt(btex $x_1$ etex scaled 1.5,1/2[1/3[a,b],1/3[c,b]]);
label.urt(btex $y_3$ etex scaled 1.5,1/2[1/3[c,b],1/3[d,b]]);
label.ulft(btex $y_2$ etex scaled 1.5,1/2[1/3[a,b],1/3[d,b]]);
label.ulft(btex $x_2$ etex scaled 1.5,1/2[1/3[a,d],1/3[c,d]]);

endfig;

beginfig(15);

pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;

p0:=1/5[1/2[c,d],b];p1:=1/4[1/2[a,c],d];
p2:=1/3[1/2[a,d],b]-(0.5,0.2)*u;p3:=1/4[1/2[a,c],b];

draw (p0-0.05*(d-c))--(p0+0.05*(d-c));
draw (p0-0.05*(b-1/2[c,d]))--(p0+0.05*(b-1/2[c,d]));
%draw (p0-0.04*(b-1/2[c,d])) withpen pencircle scaled 3bp;
%draw (p0+0.04*(b-1/2[c,d])) withpen pencircle scaled 3bp;

draw (p1-0.04*c)--(p1+0.04*c);
draw (p1-0.033*(1/2[a,c]-d))--(p1+0.033*(1/2[a,c]-d));
%draw (p1-0.03*(1/2[a,c]-d)) withpen pencircle scaled 3bp;
%draw (p1+0.03*(1/2[a,c]-d)) withpen pencircle scaled 3bp;

draw (p2-0.03*d)--(p2+0.03*d);
%draw (p2-0.1*(b-1/2[a,d]))--(p2+0.1*(b-1/2[a,d]));
draw (p2-0.08*(b-1/2[a,d])) withpen pencircle scaled 3bp;
draw (p2+0.08*(b-1/2[a,d])) withpen pencircle scaled 3bp;

draw (p3-0.04*c)--(p3+0.04*c);
%draw (p3-(0,0.3)*u)--(p3+(0,0.3)*u);
draw (p3-(0,0.22)*u) withpen pencircle scaled 3bp;
draw (p3+(0,0.22)*u) withpen pencircle scaled 3bp;




dotlabel.llft(btex $2$ etex scaled 1.8,a);
dotlabel.ulft(btex $3$ etex scaled 1.8,b);
dotlabel.lrt(btex $1$ etex scaled 1.8,c);
dotlabel.urt(btex $0$ etex scaled 1.8,d);


%draw 1/3[a,b] withpen pencircle scaled 4bp;
%draw 2/3[a,b] withpen pencircle scaled 4bp;
%draw 1/3[a,c] withpen pencircle scaled 4bp;
%draw 2/3[a,c] withpen pencircle scaled 4bp;
%draw 1/3[a,d] withpen pencircle scaled 4bp;
%draw 2/3[a,d] withpen pencircle scaled 4bp;
%draw 1/3[b,d] withpen pencircle scaled 4bp;
%draw 2/3[b,d] withpen pencircle scaled 4bp;
%draw 1/3[b,c] withpen pencircle scaled 4bp;
%draw 2/3[b,c] withpen pencircle scaled 4bp;
%draw 1/3[c,d] withpen pencircle scaled 4bp;
%draw 2/3[c,d] withpen pencircle scaled 4bp;

%draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;
%draw 1/2[2/3[b,c],2/3[b,d]] withpen pencircle scaled 4bp;
%draw 1/2[1/3[a,b],2/3[b,d]] withpen pencircle scaled 4bp;
%draw 1/2[1/3[a,d],1/3[c,d]] withpen pencircle scaled 4bp;

%singlearrow c--1/2[c,b];singlearrow c--1/2[c,a];singlearrow 1/2[a,d]--7/24[a,d];
%doublearrow a--1/2[a,b];doublearrow d--1/2[b,d];doublearrow d--1/2[d,c];

draw 1/2[a,b] withpen pencircle scaled 4bp;
draw 1/2[a,c] withpen pencircle scaled 4bp;
draw 1/2[b,c] withpen pencircle scaled 4bp;
draw 1/2[c,d] withpen pencircle scaled 4bp;
draw 1/2[a,d] withpen pencircle scaled 4bp;
draw 1/2[b,d] withpen pencircle scaled 4bp;

label.ulft(btex $y$ etex scaled 1.7,1/2[a,b]); 
label.rt(btex $y$ etex scaled 1.7,1/2[c,d]);
label.top(btex $y$ etex scaled 1.7,1/2[b,d]);
label.bot(btex $x$ etex scaled 1.7,1/2[a,c]);
label.urt(btex $x$ etex scaled 1.7,1/2[c,b]);
label.lrt(btex $x$ etex scaled 1.7,1/2[a,d]);

singlearrow c--1/3[c,b];singlearrow c--1/3[c,a];singlearrow d--1/3[d,a];
doublearrow a--1/3[a,b];doublearrow d--1/3[d,b];doublearrow d--1/3[d,c];


endfig;

beginfig(16);

pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;

draw (p0-0.05*(d-c))--(p0+0.05*(d-c));
draw (p0-0.05*(b-1/2[c,d]))--(p0+0.05*(b-1/2[c,d]));
%draw (p0-0.04*(b-1/2[c,d])) withpen pencircle scaled 3bp;
%draw (p0+0.04*(b-1/2[c,d])) withpen pencircle scaled 3bp;

draw (p1-0.04*c)--(p1+0.04*c);
%draw (p1-0.033*(1/2[a,c]-d))--(p1+0.033*(1/2[a,c]-d));
draw (p1-0.03*(1/2[a,c]-d)) withpen pencircle scaled 3bp;
draw (p1+0.03*(1/2[a,c]-d)) withpen pencircle scaled 3bp;

draw (p2-0.03*d)--(p2+0.03*d);
draw (p2-0.1*(b-1/2[a,d]))--(p2+0.1*(b-1/2[a,d]));
%draw (p2-0.08*(b-1/2[a,d])) withpen pencircle scaled 3bp;
%draw (p2+0.08*(b-1/2[a,d])) withpen pencircle scaled 3bp;

draw (p3-0.04*c)--(p3+0.04*c);
%draw (p3-(0,0.3)*u)--(p3+(0,0.3)*u);
draw (p3-(0,0.22)*u) withpen pencircle scaled 3bp;
draw (p3+(0,0.22)*u) withpen pencircle scaled 3bp;

dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.ulft(btex $3$ etex scaled 1.8,b);
dotlabel.lrt(btex $1$ etex scaled 1.8,c);
dotlabel.urt(btex $2$ etex scaled 1.8,d);

%draw 1/3[a,b] withpen pencircle scaled 4bp;
%draw 2/3[a,b] withpen pencircle scaled 4bp;
%draw 1/3[a,c] withpen pencircle scaled 4bp;
%draw 2/3[a,c] withpen pencircle scaled 4bp;
%draw 1/3[a,d] withpen pencircle scaled 4bp;
%draw 2/3[a,d] withpen pencircle scaled 4bp;
%draw 1/3[b,d] withpen pencircle scaled 4bp;
%draw 2/3[b,d] withpen pencircle scaled 4bp;
%draw 1/3[b,c] withpen pencircle scaled 4bp;
%draw 2/3[b,c] withpen pencircle scaled 4bp;
%draw 1/3[c,d] withpen pencircle scaled 4bp;
%draw 2/3[c,d] withpen pencircle scaled 4bp;

%draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;
%draw 1/2[2/3[b,c],2/3[b,d]] withpen pencircle scaled 4bp;
%draw 1/2[1/3[a,b],2/3[b,d]] withpen pencircle scaled 4bp;
%draw 1/2[1/3[a,d],1/3[c,d]] withpen pencircle scaled 4bp;

%singlearrow a--1/2[a,b];singlearrow a--1/2[a,c];singlearrow d--1/2[d,b];
%doublearrow a--7/24[a,d];doublearrow c--1/2[b,c];doublearrow c--1/2[c,d];

draw 1/2[a,b] withpen pencircle scaled 4bp;
draw 1/2[a,c] withpen pencircle scaled 4bp;
draw 1/2[b,c] withpen pencircle scaled 4bp;
draw 1/2[c,d] withpen pencircle scaled 4bp;
draw 1/2[a,d] withpen pencircle scaled 4bp;
draw 1/2[b,d] withpen pencircle scaled 4bp;

label.ulft(btex $x$ etex scaled 1.7,1/2[a,b]); 
label.rt(btex $y$ etex scaled 1.7,1/2[c,d]);
label.top(btex $x$ etex scaled 1.7,1/2[b,d]);
label.bot(btex $x$ etex scaled 1.7,1/2[a,c]);
label.urt(btex $y$ etex scaled 1.7,1/2[c,b]);
label.lrt(btex $y$ etex scaled 1.7,1/2[a,d]);

singlearrow a--1/3[a,b];singlearrow a--1/3[a,c];singlearrow d--1/3[d,b];
doublearrow a--1/3[a,d];doublearrow c--1/3[c,b];doublearrow c--1/3[c,d];

endfig;

beginfig(17);

pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;

p0:=1/5[1/2[c,d],b];p1:=1/4[1/2[a,c],d];
p2:=1/3[1/2[a,d],b]-(0.5,0.2)*u;p3:=1/4[1/2[a,c],b];

draw (p0-0.05*(d-c))--(p0+0.05*(d-c));
%draw (p0-0.05*(b-1/2[c,d]))--(p0+0.05*(b-1/2[c,d]));
draw (p0-0.04*(b-1/2[c,d])) withpen pencircle scaled 3bp;
draw (p0+0.04*(b-1/2[c,d])) withpen pencircle scaled 3bp;

draw (p1-0.04*c)--(p1+0.04*c);
draw (p1-0.033*(1/2[a,c]-d))--(p1+0.033*(1/2[a,c]-d));
%draw (p1-0.03*(1/2[a,c]-d)) withpen pencircle scaled 3bp;
%draw (p1+0.03*(1/2[a,c]-d)) withpen pencircle scaled 3bp;

draw (p2-0.03*d)--(p2+0.03*d);
draw (p2-0.1*(b-1/2[a,d]))--(p2+0.1*(b-1/2[a,d]));
%draw (p2-0.08*(b-1/2[a,d])) withpen pencircle scaled 3bp;
%draw (p2+0.08*(b-1/2[a,d])) withpen pencircle scaled 3bp;

draw (p3-0.04*c)--(p3+0.04*c);
%draw (p3-(0,0.3)*u)--(p3+(0,0.3)*u);
draw (p3-(0,0.22)*u) withpen pencircle scaled 3bp;
draw (p3+(0,0.22)*u) withpen pencircle scaled 3bp;

label.ulft(btex $0$ etex scaled 1.8,a+(0,0.1)*u);
label.llft(btex $1$ etex scaled 1.8,b-(0.3,0.1)*u);
label.urt(btex $2$ etex scaled 1.8,c+(0.2,0.1)*u);
label.lrt(btex $3$ etex scaled 1.8,d-(0,0.1)*u);

dotlabel.llft(btex $\alpha^{-1}N$ etex scaled 1.8,a);
dotlabel.ulft(btex $N$ etex scaled 1.8,b);
dotlabel.lrt(btex $\alpha N$ etex scaled 1.8,c);
dotlabel.urt(btex $\alpha^2N$ etex scaled 1.8,d);


%draw 1/3[a,b] withpen pencircle scaled 4bp;
%draw 2/3[a,b] withpen pencircle scaled 4bp;
%draw 1/3[a,c] withpen pencircle scaled 4bp;
%draw 2/3[a,c] withpen pencircle scaled 4bp;
%draw 1/3[a,d] withpen pencircle scaled 4bp;
%draw 2/3[a,d] withpen pencircle scaled 4bp;
%draw 1/3[b,d] withpen pencircle scaled 4bp;
%draw 2/3[b,d] withpen pencircle scaled 4bp;
%draw 1/3[b,c] withpen pencircle scaled 4bp;
%draw 2/3[b,c] withpen pencircle scaled 4bp;
%draw 1/3[c,d] withpen pencircle scaled 4bp;
%draw 2/3[c,d] withpen pencircle scaled 4bp;

%draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;
%draw 1/2[2/3[b,c],2/3[b,d]] withpen pencircle scaled 4bp;
%draw 1/2[1/3[a,b],2/3[b,d]] withpen pencircle scaled 4bp;
%draw 1/2[1/3[a,d],1/3[c,d]] withpen pencircle scaled 4bp;

%singlearrow a--1/2[a,b];singlearrow b--1/2[b,c];singlearrow c--1/2[c,d];
%doublearrow a--7/24[a,d];whitearrow a--1/2[a,c];whitearrow b--1/2[b,d];

draw 1/2[a,b] withpen pencircle scaled 4bp;
draw 1/2[a,c] withpen pencircle scaled 4bp;
draw 1/2[b,c] withpen pencircle scaled 4bp;
draw 1/2[c,d] withpen pencircle scaled 4bp;
draw 1/2[a,d] withpen pencircle scaled 4bp;
draw 1/2[b,d] withpen pencircle scaled 4bp;

label.ulft(btex $x$ etex scaled 1.7,1/2[a,b]); 
label.rt(btex $x$ etex scaled 1.7,1/2[c,d]);
label.top(btex $y$ etex scaled 1.7,1/2[b,d]);
label.bot(btex $y$ etex scaled 1.7,1/2[a,c]);
label.urt(btex $x$ etex scaled 1.7,1/2[c,b]);
label.lrt(btex $z$ etex scaled 1.7,1/2[a,d]);

singlearrow a--1/3[a,b];singlearrow b--1/3[b,c];singlearrow c--1/3[c,d];
whitearrow a--1/3[a,d];doublearrow a--1/3[a,c];doublearrow b--1/3[b,d];

endfig;

beginfig(18);

pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;

p0:=1/5[1/2[c,d],b];p1:=1/4[1/2[a,c],d];
p2:=1/3[1/2[a,d],b]-(0.5,0.2)*u;p3:=1/4[1/2[a,c],b];

draw (p0-0.05*(d-c))--(p0+0.05*(d-c));
draw (p0-0.05*(b-1/2[c,d]))--(p0+0.05*(b-1/2[c,d]));
%draw (p0-0.04*(b-1/2[c,d])) withpen pencircle scaled 3bp;
%draw (p0+0.04*(b-1/2[c,d])) withpen pencircle scaled 3bp;

draw (p1-0.04*c)--(p1+0.04*c);
draw (p1-0.033*(1/2[a,c]-d))--(p1+0.033*(1/2[a,c]-d));
%draw (p1-0.03*(1/2[a,c]-d)) withpen pencircle scaled 3bp;
%draw (p1+0.03*(1/2[a,c]-d)) withpen pencircle scaled 3bp;

draw (p2-0.03*d)--(p2+0.03*d);
draw (p2-0.1*(b-1/2[a,d]))--(p2+0.1*(b-1/2[a,d]));
%draw (p2-0.08*(b-1/2[a,d])) withpen pencircle scaled 3bp;
%draw (p2+0.08*(b-1/2[a,d])) withpen pencircle scaled 3bp;

draw (p3-0.04*c)--(p3+0.04*c);
draw (p3-(0,0.3)*u)--(p3+(0,0.3)*u);
%draw (p3-(0,0.22)*u) withpen pencircle scaled 3bp;
%draw (p3+(0,0.22)*u) withpen pencircle scaled 3bp;

label.ulft(btex $0$ etex scaled 1.8,a+(0,0.1)*u);
label.llft(btex $3$ etex scaled 1.8,b-(0.3,0.1)*u);
label.urt(btex $2$ etex scaled 1.8,c+(0.2,0.1)*u);
label.lrt(btex $1$ etex scaled 1.8,d-(0,0.1)*u);

dotlabel.llft(btex $\alpha^{-1}N$ etex scaled 1.8,a);
dotlabel.ulft(btex $N$ etex scaled 1.8,b);
dotlabel.lrt(btex $\alpha N$ etex scaled 1.8,c);
dotlabel.urt(btex $\alpha^2N$ etex scaled 1.8,d);

%draw 1/3[a,b] withpen pencircle scaled 4bp;
%draw 2/3[a,b] withpen pencircle scaled 4bp;
%draw 1/3[a,c] withpen pencircle scaled 4bp;
%draw 2/3[a,c] withpen pencircle scaled 4bp;
%draw 1/3[a,d] withpen pencircle scaled 4bp;
%draw 2/3[a,d] withpen pencircle scaled 4bp;
%draw 1/3[b,d] withpen pencircle scaled 4bp;
%draw 2/3[b,d] withpen pencircle scaled 4bp;
%draw 1/3[b,c] withpen pencircle scaled 4bp;
%draw 2/3[b,c] withpen pencircle scaled 4bp;
%draw 1/3[c,d] withpen pencircle scaled 4bp;
%draw 2/3[c,d] withpen pencircle scaled 4bp;

%draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;
%draw 1/2[2/3[b,c],2/3[b,d]] withpen pencircle scaled 4bp;
%draw 1/2[1/3[a,b],2/3[b,d]] withpen pencircle scaled 4bp;
%draw 1/2[1/3[a,d],1/3[c,d]] withpen pencircle scaled 4bp;

%singlearrow a--7/24[a,d];singlearrow c--1/2[c,b];singlearrow d--1/2[c,d];
%doublearrow a--1/2[a,b];
%whitearrow a--1/2[a,c] withpen pencircle scaled 1;whitearrow d--1/2[d,b] withpen pencircle scaled 1;

draw 1/2[a,b] withpen pencircle scaled 4bp;
draw 1/2[a,c] withpen pencircle scaled 4bp;
draw 1/2[b,c] withpen pencircle scaled 4bp;
draw 1/2[c,d] withpen pencircle scaled 4bp;
draw 1/2[a,d] withpen pencircle scaled 4bp;
draw 1/2[b,d] withpen pencircle scaled 4bp;

label.ulft(btex $z$ etex scaled 1.7,1/2[a,b]); 
label.rt(btex $x$ etex scaled 1.7,1/2[c,d]);
label.top(btex $y$ etex scaled 1.7,1/2[b,d]);
label.bot(btex $y$ etex scaled 1.7,1/2[a,c]);
label.urt(btex $x$ etex scaled 1.7,1/2[c,b]);
label.lrt(btex $x$ etex scaled 1.7,1/2[a,d]);

singlearrow a--1/3[a,d];singlearrow c--1/3[c,b];singlearrow d--1/3[d,c];
whitearrow a--1/3[a,b];doublearrow a--1/3[a,c];doublearrow d--1/3[d,b];

endfig;

beginfig(19);
pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw a--c;

dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.top(btex $1$ etex scaled 1.8,b);
dotlabel.lrt(btex $2$ etex scaled 1.8,c);


draw 1/3[a,b] withpen pencircle scaled 4bp;
draw 2/3[a,b] withpen pencircle scaled 4bp;
draw 1/3[a,c] withpen pencircle scaled 4bp;
draw 2/3[a,c] withpen pencircle scaled 4bp;
draw 1/3[b,c] withpen pencircle scaled 4bp;
draw 2/3[b,c] withpen pencircle scaled 4bp;

draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;

label.ulft(btex $a$ etex scaled 1.5,2/3[a,b]);
label.urt(btex $b$ etex scaled 1.5,2/3[c,b]);
label.ulft(btex $c$ etex scaled 1.5,1/3[a,b]);
label.top(btex $d$ etex scaled 1.5,1/2[1/3[a,b],1/3[c,b]]);
label.urt(btex $e$ etex scaled 1.5,2/3[b,c]);
label.top(btex $f$ etex scaled 1.5,1/3[a,c]);
label.top(btex $g$ etex scaled 1.5,2/3[a,c]);

endfig;

beginfig(20);
pickup pencircle scaled 1.5pt;

dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.top(btex $1$ etex scaled 1.8,b);
dotlabel.lrt(btex $2$ etex scaled 1.8,c);

draw 1/4[a,b]--3/4[a,b];draw 3/4[a,b]--1/4[b,c];draw 1/4[b,c]--3/4[b,c];
draw 1/4[a,b]--1/4[a,c];draw 1/4[a,c]--3/4[a,c];draw 3/4[a,c]--1/4[c,b];

draw a--1/4[a,b] dashed evenly scaled 1;
draw a--1/4[a,c] dashed evenly scaled 1;
draw b--1/4[b,a] dashed evenly scaled 1;
draw b--1/4[b,c] dashed evenly scaled 1;
draw c--1/4[c,a] dashed evenly scaled 1;
draw c--1/4[c,b] dashed evenly scaled 1;

singlearrow 1/4[a,b]--1/2[a,b];
singlearrow 1/4[b,c]--1/2[b,c];
singlearrow 1/4[a,c]--1/2[a,c];

singlearrow 1/4[a,b]--1/2[1/4[a,b],1/4[a,c]];
singlearrow 1/4[b,a]--1/2[1/4[b,a],1/4[b,c]];
singlearrow 1/4[c,a]--1/2[1/4[c,a],1/4[c,b]];

label.ulft(btex $q_{01}$ etex scaled 1.5,1/2[a,b]);
label.urt(btex $q_{12}$ etex scaled 1.5,1/2[b,c]);
label.top(btex $q_{02}$ etex scaled 1.5,1/2[a,c]);

label.urt(btex $\alpha^0_{12}$ etex scaled 1.5,1/2[1/4[a,b],1/4[a,c]]);
label.ulft(btex $\alpha^0_{12}$ etex scaled 1.5,1/2[1/4[c,a],1/4[c,b]]);
label.bot(btex $\alpha^1_{02}$ etex scaled 1.5,1/2[1/4[b,a],1/4[b,c]]);

endfig;


beginfig(21);
%pickup pencircle scaled 1.5pt;
pair P[]; pair Q[];
P1:=(2,0)*u;P2:=(0,2)*u;P3:=(-2,0)*u;P4:=(0,-2)*u;
Q1:=dir(60)*2*u;Q2:=dir(160)*2*u;Q3:=dir(-150)*2*u;Q4:=dir(-10)*2*u;
draw P1..P2..P3..P4..P1 dashed evenly;
draw Q1--Q2;draw Q3--Q4;draw Q1--Q3;draw Q1--Q4;draw Q2--Q3;draw Q2--Q4;
label.rt(btex $c$ etex,1/2[Q2,Q3]);
label.top(btex $a$ etex,1/2[Q1,Q2]);
label.bot(btex $b$ etex,1/2[Q3,Q4]);
label.lft(btex $d$ etex,1/2[Q1,Q4]);
label.rt(btex $e$ etex,1/4[Q3,Q1]);
label.top(btex $f$ etex,1/2[Q2,Q4]);

endfig;

beginfig(22);
pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;

dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.ulft(btex $1$ etex scaled 1.8,b);
dotlabel.lrt(btex $2$ etex scaled 1.8,c);
dotlabel.urt(btex $3$ etex scaled 1.8,d);

label.lft(btex $z$ etex scaled 1.8,1/2[a,b]);
label.rt(btex $z$ etex scaled 1.8,1/2[c,d]);
label.urt(btex $z^\prime$ etex scaled 1.8,1/2[b,c]);
label.rt(btex $z^\prime$ etex scaled 1.8,1/3[a,d]);
label.top(btex $z^{\prime\prime}$ etex scaled 1.8,1/2[b,d]);
label.bot(btex $z^{\prime\prime}$ etex scaled 1.8,1/2[a,c]);

endfig;

end;





==> draws/SLrepFigures_ <==
u:=1cm;
pair cuta[];
cuta0:=(0,0);cuta2:=u*dir(0);cuta1:=u*dir(60);cuta3:=cuta1+cuta2;
pair cutb[];
 for i=0 upto 4:
  cutb[i]:=cuta[i]+dir(60)*3u;
 endfor;
pair cutc[];
 for i=0 upto 4:
  cutc[i]:=cuta[i]+dir(0)*3u;
 endfor;
pair cutd[];
for i=0 upto 4:
  cutd[i]:=cutc[i]+dir(60)*3u;
 endfor;

pair a;pair b; pair c; pair d; pair ds;
a:=cuta0;b:=cuta1+dir(60)*5u;c:=cuta2+dir(0)*5u;ds:=cuta3+dir(0)*5*u+dir(60)*5u;d:=ds-(1.4*u,-0.5*u);

path ee[];pair CC;ee1:=a--1/2[b,c];ee2:=b--1/2[a,c];CC:=ee1 intersectionpoint ee2;

input cmarrows;

setup_cmarrows(
  arrow_name     = "twoheadarrow";
  parameter_file = "cmr25.mf";
  macro_name     = "doublearrow");

setup_cmarrows(
  arrow_name     = "shortaxisarrow";
  parameter_file = "cmr25.mf";
  macro_name     = "singlearrow");

setup_cmarrows(
  arrow_name     = "shortaxisarrow";
  parameter_file = "cmr10.mf";
  macro_name     = "smallsinglearrow");


def whitearrow expr p = _apth:=p; _finwhitearr enddef;

  def _finwhitearr text t =
    draw _apth t;
    fill arrowhead _apth  t withcolor white;
    draw arrowhead _apth  t
  enddef;


%example: doublearrow (60pt,10pt)--(95pt,45pt);


beginfig(1);
pickup pencircle scaled 1.5pt;
draw a--c; draw b--c; draw c--d;
draw b--d; draw a--c; draw a--b;
draw a--0.52*d; draw 0.58*d--d;
dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.ulft(btex $1$ etex scaled 1.8,b);
dotlabel.lrt(btex $2$ etex scaled 1.8,c);
dotlabel.urt(btex $3$ etex scaled 1.8,d);
%label.lft(btex $c_{01}$ etex scaled 1.8,1/2[a,b]);
%label.rt(btex $c_{23}$ etex scaled 1.8,1/2[c,d]);
%label.ulft(btex $c_{03}$ etex scaled 1.8,1/2[a,d]);
%label.rt(btex $c_{12}$ etex scaled 1.8,1/2[b,c]+(0.1*u,0));
%label.bot(btex $c_{02}$ etex scaled 1.8,1/2[a,c]);
%label.top(btex $c_{13}$ etex scaled 1.8,1/2[b,d]);

draw 1/2[a,b] withpen pencircle scaled 4bp;
draw 1/2[c,d] withpen pencircle scaled 4bp;
draw 1/2*d withpen pencircle scaled 4bp;
draw 1/2[b,c] withpen pencircle scaled 4bp;
draw 1/2[a,c] withpen pencircle scaled 4bp;
draw 1/2[b,d] withpen pencircle scaled 4bp;

endfig;


beginfig(2);

pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;

dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.ulft(btex $1$ etex scaled 1.8,b);
dotlabel.lrt(btex $2$ etex scaled 1.8,c);
dotlabel.urt(btex $3$ etex scaled 1.8,d);

draw 1/3[a,b] withpen pencircle scaled 4bp;
draw 2/3[a,b] withpen pencircle scaled 4bp;
draw 1/3[a,c] withpen pencircle scaled 4bp;
draw 2/3[a,c] withpen pencircle scaled 4bp;
draw 1/3[a,d] withpen pencircle scaled 4bp;
draw 2/3[a,d] withpen pencircle scaled 4bp;
draw 1/3[b,d] withpen pencircle scaled 4bp;
draw 2/3[b,d] withpen pencircle scaled 4bp;
draw 1/3[b,c] withpen pencircle scaled 4bp;
draw 2/3[b,c] withpen pencircle scaled 4bp;
draw 1/3[c,d] withpen pencircle scaled 4bp;
draw 2/3[c,d] withpen pencircle scaled 4bp;

draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;
draw 1/2[2/3[b,c],2/3[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/3[a,b],2/3[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/3[a,d],1/3[c,d]] withpen pencircle scaled 4bp;

draw 1/3[a,b]--2/3[b,c] dashed evenly;
draw 1/3[a,b]--2/3[b,d] dashed evenly;
draw 1/3[c,b]--1/3[d,b] dashed evenly;

endfig;

beginfig(3);

pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;

dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.ulft(btex $1$ etex scaled 1.8,b);
dotlabel.lrt(btex $2$ etex scaled 1.8,c);
dotlabel.urt(btex $3$ etex scaled 1.8,d);

draw 1/2[a,b] withpen pencircle scaled 4bp;
draw 1/2[a,c] withpen pencircle scaled 4bp;
draw 1/2[a,d] withpen pencircle scaled 4bp;
draw 1/2[b,c] withpen pencircle scaled 4bp;
draw 1/2[b,d] withpen pencircle scaled 4bp;
draw 1/2[c,d] withpen pencircle scaled 4bp;

draw 1/4[a,b] withpen pencircle scaled 4bp;
draw 1/4[a,c] withpen pencircle scaled 4bp;
draw 1/4[a,d] withpen pencircle scaled 4bp;
draw 1/4[b,c] withpen pencircle scaled 4bp;
draw 1/4[b,d] withpen pencircle scaled 4bp;
draw 1/4[c,d] withpen pencircle scaled 4bp;

draw 3/4[a,b] withpen pencircle scaled 4bp;
draw 3/4[a,c] withpen pencircle scaled 4bp;
draw 3/4[a,d] withpen pencircle scaled 4bp;
draw 3/4[b,c] withpen pencircle scaled 4bp;
draw 3/4[b,d] withpen pencircle scaled 4bp;
draw 3/4[c,d] withpen pencircle scaled 4bp;

draw 1/2[1/2[b,c],1/2[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/2[b,c],1/2[c,d]] withpen pencircle scaled 4bp;
draw 1/2[1/2[b,d],1/2[c,d]] withpen pencircle scaled 4bp;

draw 1/2[1/2[a,c],1/2[c,d]] withpen pencircle scaled 4bp;
draw 1/2[1/2[a,d],1/2[c,d]] withpen pencircle scaled 4bp;
draw 1/2[1/2[a,c],1/2[a,d]] withpen pencircle scaled 4bp;

draw 1/2[1/2[a,b],1/2[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/2[a,d],1/2[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/2[a,b],1/2[a,d]] withpen pencircle scaled 4bp;

draw 1/2[1/2[a,b],1/2[b,c]] withpen pencircle scaled 4bp;
draw 1/2[1/2[a,c],1/2[b,c]] withpen pencircle scaled 4bp;
draw 1/2[1/2[a,b],1/2[a,c]] withpen pencircle scaled 4bp;

draw 1/2[(1/2[1/2[a,b],1/2[a,d]]),(1/2[1/2[b,c],1/2[c,d]])] withpen pencircle scaled 4bp;

draw 1/2[1/2[a,b],1/2[a,c]]--3/4[b,c] dashed evenly;
draw 3/4[b,c]--1/2[1/2[b,d],1/2[c,d]] dashed evenly;
draw 1/2[1/2[a,b],1/2[a,c]]--1/2[1/2[b,d],1/2[c,d]] dashed evenly;
draw 1/2[1/2[a,b],1/2[a,c]]--1/4[b,c] dashed evenly;
draw 1/4[b,c]--1/2[1/2[b,d],1/2[c,d]] dashed evenly;

endfig;

beginfig(4);
pickup pencircle scaled 1.5pt;

draw a--b--c--a;

pair Q; Q:=d;

draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;

draw 1/3[a,b] withpen pencircle scaled 4bp;
draw 2/3[a,b] withpen pencircle scaled 4bp;
draw 1/3[a,c] withpen pencircle scaled 4bp;
draw 2/3[a,c] withpen pencircle scaled 4bp;
draw 1/3[b,c] withpen pencircle scaled 4bp;
draw 2/3[b,c] withpen pencircle scaled 4bp;

draw 1/3[a,b]--1/3[c,b] dashed evenly;
draw 1/3[a,c]--1/3[b,c] dashed evenly;
draw 1/3[b,a]--1/3[c,a] dashed evenly;

dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.top(btex $1$ etex scaled 1.8,b);
dotlabel.lrt(btex $2$ etex scaled 1.8,c);

endfig;


beginfig(5);
pickup pencircle scaled 1.5pt;

draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;


draw 1/3[a,b] withpen pencircle scaled 4bp;
draw 2/3[a,b] withpen pencircle scaled 4bp;
draw 1/3[a,c] withpen pencircle scaled 4bp;
draw 2/3[a,c] withpen pencircle scaled 4bp;
draw 1/3[a,d] withpen pencircle scaled 4bp;
draw 2/3[a,d] withpen pencircle scaled 4bp;
draw 1/3[b,d] withpen pencircle scaled 4bp;
draw 2/3[b,d] withpen pencircle scaled 4bp;
draw 1/3[b,c] withpen pencircle scaled 4bp;
draw 2/3[b,c] withpen pencircle scaled 4bp;
draw 1/3[c,d] withpen pencircle scaled 4bp;
draw 2/3[c,d] withpen pencircle scaled 4bp;

draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;
draw 1/2[2/3[b,c],2/3[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/3[a,b],2/3[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/3[a,d],1/3[c,d]] withpen pencircle scaled 4bp;

draw 1/3[b,a]--1/3[c,a] dashed evenly;
draw 1/3[c,a]--1/3[d,a] dashed evenly;
draw 1/3[d,a]--1/3[b,a] dashed evenly;

dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.ulft(btex $1$ etex scaled 1.8,b);
dotlabel.lrt(btex $2$ etex scaled 1.8,c);
dotlabel.urt(btex $3$ etex scaled 1.8,d);

endfig;

beginfig(6);
pair a[]; pair e[];

pickup pencircle scaled 0.4pt;

a6:=(0,0);a1:=(0.4,1.4)*u;a2:=(1.4,1.4)*u;
a3:=(0,1)*u;a4:=(1,1)*u;a5:=(1.4,0.5)*u;a7:=(1,0)*u;
e1:=1/2[a1,a2];e2:=1/2[a3,a1];e3:=1/2[a4,a2];e4:=1/2[a3,a4];e5:=1/2[a3,a6];
e6:=1/2[a4,a7];e7:=1/2[a2,a5];e8:=1/2[a6,a7];e9:=1/2[a5,a7];

draw a3--a4--a7--a6--a3--a1--a2--a5--a7--a4--a2;

draw e5--e6--e7;draw e8--e4--e1;draw e2--e3--e9;

draw a6--a4--a1;draw a7--a3--a2;draw a2--a7;draw a5--a4;

endfig;

beginfig(7);

pair a[];
a1:=(0,0);a2:=(0,1)*u;a3:=(1,0)*u;;

whitearrow a1--a2 withpen pencircle scaled 1bp;
doublearrow a1--a3 withpen pencircle scaled 1bp;
singlearrow  a2--a3 withpen pencircle scaled 1bp;

endfig;

beginfig(8);%truncated simplex with labelings.

pickup pencircle scaled 1pt;

draw cuta0--cuta1 dashed evenly scaled 1;
draw cuta0--cuta2 dashed evenly scaled 1;
smallsinglearrow  cuta1--1/2[cuta1,cuta3] withpen pencircle scaled 1bp;draw 1/2[cuta1,cuta3]--cuta3;
smallsinglearrow  cuta2--1/2[cuta3,cuta2] withpen pencircle scaled 1bp;draw 1/2[cuta3,cuta2]--cuta3;
smallsinglearrow  cuta1--1/2[cuta2,cuta1] withpen pencircle scaled 1bp;draw 1/2[cuta2,cuta1]--cuta2;
draw cuta0--0.4*cuta3 dashed evenly scaled 1;
draw 0.6*cuta3--cuta3 dashed evenly scaled 1;

dotlabel.llft(btex $0$ etex scaled 1.3,cuta0);
dotlabel.ulft(btex $1$ etex scaled 1.3,cutb1);
dotlabel.lrt(btex $2$ etex scaled 1.3,cutc2);
dotlabel.urt(btex $3$ etex scaled 1.3,cutd3);
dotlabel.urt(btex $$ etex,cuta2);
dotlabel.rt(btex $$ etex,cuta3);
dotlabel.lft(btex $$ etex,cuta1);
dotlabel.lft(btex $$ etex,cutb0);
dotlabel.rt(btex $$ etex,cutb2);
dotlabel.top(btex $$ etex,cutb3);
dotlabel.bot(btex $$ etex,cutc0);
dotlabel.lft(btex $$ etex,cutc1);
dotlabel.rt(btex $$ etex,cutc3);
dotlabel.lft(btex $$ etex,cutd0);
dotlabel.top(btex $$ etex,cutd1);
dotlabel.rt(btex $$ etex,cutd2);

draw cutb0--cutb1 dashed evenly scaled 1;
draw cutb1--cutb3 dashed evenly scaled 1;
smallsinglearrow  cutb2--1/2[cutb2,cutb3] withpen pencircle scaled 1pt;draw 1/2[cutb2,cutb3]--cutb3; 
smallsinglearrow  cutb0--1/2[cutb0,cutb2] withpen pencircle scaled 1pt;draw 1/2[cutb0,cutb2]--cutb2;
draw cutb1--cutb2 dashed evenly scaled 1;
smallsinglearrow  cutb0--3/4[cutb0,(cutb0+0.4*cuta3)] withpen pencircle scaled 1pt;
draw 3/4[cutb0,(cutb0+0.4*cuta3)]--(cutb0+0.4*cuta3);
draw (cutb0+0.6*cuta3)--cutb3;

smallsinglearrow  cutc0--1/2[cutc1,cutc0] withpen pencircle scaled 1pt;draw 1/2[cutc1,cutc0]--cutc1;
smallsinglearrow  cutc1--1/2[cutc1,cutc3] withpen pencircle scaled 1pt;draw 1/2[cutc1,cutc3]--cutc3;
draw cutc2--cutc3 dashed evenly scaled 1;
draw cutc0--cutc2 dashed evenly scaled 1;
draw cutc1--cutc2 dashed evenly scaled 1;
draw cutc0--(cutc0+0.4*cuta3);
smallsinglearrow  (cutc0+0.6*cuta3)--1/2[(cutc0+0.6*cuta3),cutc3] withpen pencircle scaled 1.2pt;
draw 1/2[(cutc0+0.6*cuta3),cutc3]--cutc3;

smallsinglearrow  cutd0--1/2[cutd0,cutd1] withpen pencircle scaled 1pt;draw 1/2[cutd0,cutd1]--cutd1; 
draw cutd1--cutd3 dashed evenly scaled 1;
draw cutd2--cutd3 dashed evenly scaled 1;
smallsinglearrow  cutd0--1/2[cutd2,cutd0] withpen pencircle scaled 1pt;draw 1/2[cutd2,cutd0]--cutd2;
smallsinglearrow  cutd1--2/3[cutd1,cutd2] withpen pencircle scaled 1pt;draw 2/3[cutd1,cutd2]--cutd2;
draw cutd0--(cutd0+0.4*cuta3) dashed evenly scaled 1;
draw (cutd0+0.6*cuta3)--cutd3 dashed evenly scaled 1;
smallsinglearrow  cuta3--2/3[cuta3,0.4*cutd3] withpen pencircle scaled 1pt;draw 2/3[cuta3,0.4*cutd3]--0.4*cutd3;
draw (0.6*cutd3)--cutd0;

smallsinglearrow  cutb2--1/2[cutb2,cutc1] withpen pencircle scaled 1pt;draw 1/2[cutb2,cutc1]--cutc1;
smallsinglearrow  cuta1--1/2[cuta1,cutb0] withpen pencircle scaled 1pt;draw 1/2[cuta1,cutb0]--cutb0;
smallsinglearrow  cutc3--1/2[cutd2,cutc3] withpen pencircle scaled 1pt;draw 1/2[cutd2,cutc3]--cutd2;
smallsinglearrow  cutb3--1/2[cutd1,cutb3] withpen pencircle scaled 1pt;draw 1/2[cutd1,cutb3]--cutd1;
smallsinglearrow  cuta2--1/2[cutc0,cuta2] withpen pencircle scaled 1pt;draw 1/2[cutc0,cuta2]--cutc0;


label.bot(btex $q_{02}$ etex,1/2[cuta2,cutc0]);
label.lft(btex $q_{01}$ etex,1/2[cutb0,cuta1]);
label.rt(btex $q_{12}$ etex,1/2[cutb2,cutc1]);
label.rt(btex $q_{23}$ etex,1/2[cutc3,cutd2]);
label.top(btex $q_{13}$ etex,1/2[cutb3,cutd1]);
label.rt(btex $q_{03}$ etex,2/3[cuta3,0.4*cutd3]-u*(0,0.08));

label.lft(btex $\alpha^0_{12}$ etex,2/3[cuta0,cuta1]-(0.08,0)*u);
label.top(btex $\alpha^0_{13}$ etex,1/2[cuta3,cuta1]);
label.rt(btex $\alpha^0_{23}$ etex,1/2[cuta3,cuta2]);

label.bot(btex $\alpha^1_{02}$ etex,1/2[cutb0,cutb2]);
label.rt(btex $\alpha^1_{23}$ etex,1/2[cutb2,cutb3]);
label.lft(btex $\alpha^1_{03}$ etex,1/2[cutb0,cutb1]-(0.08,0)*u);

label.lft(btex $\alpha^2_{01}$ etex,1/2[cutc0,cutc1]);
label.top(btex $\alpha^2_{13}$ etex,1/2[cutc3,cutc1]);
label.rt(btex $\alpha^2_{03}$ etex,5/8[cutc2,cutc3]);

label.lft(btex $\alpha^3_{01}$ etex,1/2[cutd0,cutd1]);
label.bot(btex $\alpha^3_{02}$ etex,1/2[cutd2,cutd0]-u*(0.1,0));
label.rt(btex $\alpha^3_{12}$ etex,1/3[cutd2,cutd3]);

endfig;

beginfig(9);
numeric n;n:=7;

pickup pencircle scaled 1pt;

label.llft(btex $i$ etex scaled 1.2,a);
label.top(btex $j$ etex scaled 1.2,b);
label.lrt(btex $k$ etex scaled 1.2,c);

pair p[];path l[];

p1:=(n-1)/n*b;p2:=(n-2)/n*b;p3:=(n-3)/n*b;
p4:=p1+1/n*c;p5:=p2+1/n*c;p6:=p3+1/n*c;

p7:=CC-(0.3,0.3)*u;p8:=p7+1/n*b;p9:=p7+1/n*c;p10:=p9+1/n*b;

p11:=1/n*b;p12:=1/n*c;p13:=p12+1/n*b;
p14:=(n-1)/n*c;p15:=(n-2)/n*c;p16:=p14+1/n*b;p17:=p15+1/n*b;

p18:=p5+1/n*c;p19:=p6+1/n*c;

l1:=p1--p4;l2:=p2--p18;l3:=p3--p19+(0.4,0)*u;
l4:=p8-(0.4,0)*u--p10+(0.4,0)*u;l5:=p7-(0.4,0)*u--p9+(0.4,0)*u;
l6:=p4--p6+dir(-120)*0.4u;l7:=p18--p19+dir(-120)*0.4u;
l8:=p8+dir(60)*0.4u--p7+dir(-120)*0.4u;l9:=p10+dir(60)*0.4u--p9+dir(-120)*0.4u;

l10:=p11--p13+(0.4,0)*u;l11:=p17-(0.4,0)*u--p16;
l12:=p13+dir(60)*0.4u--p12;l13:=p17+dir(60)*0.4u--p15;l14:=p16--p14;


pickup pencircle scaled 1.5pt;

%draw CC withpen pencircle scaled 2.5bp;

%p11:=((p1 shifted -CC) rotated 120) shifted CC;


for i=1 upto 19:
  draw p[i] withpen pencircle scaled 2.5bp;
endfor;

label.ulft(btex $(1,1)$ etex scaled 0.9,p5+(0.20,0.13)*u);
label.ulft(btex $(1,n-1)$ etex scaled 0.9,p12+(0.78,0.13)*u);
label.ulft(btex $(1,2)$ etex scaled 0.9,p6+(0.20,0.13)*u);
label.ulft(btex $(2,1)$ etex scaled 0.9,p19+(0.20,0.13)*u);
label.ulft(btex $(r,s)$ etex scaled 0.9,p9+(0.20,0.13)*u);
label.ulft(btex $(n-1,1)$ etex scaled 0.9,p14+(0.6,0.13)*u);

draw a--b--c--a;

for i=1 upto 11:
  draw l[i] dashed evenly scaled 1;
endfor;

draw subpath(0,0.45) of l12 dashed evenly scaled 1;draw subpath(0.85,1) of l12 dashed evenly scaled 1;
draw subpath(0,0.45) of l13 dashed evenly scaled 1;draw subpath(0.85,1) of l13 dashed evenly scaled 1;
draw subpath(0,0.22) of l14 dashed evenly scaled 1;draw subpath(0.8,1) of l14 dashed evenly scaled 1;

dotlabel.lrt(btex $b$ etex scaled 1,p7);
dotlabel.ulft(btex $c$ etex scaled 1,p8);
dotlabel.lrt(btex $d$ etex scaled 1,p9);
dotlabel.ulft(btex $a$ etex scaled 1,p10);

endfig;

beginfig(10);
label.llft(btex $i$ etex scaled 1.2,a);
label.top(btex $j$ etex scaled 1.2,b);
label.lrt(btex $k$ etex scaled 1.2,c);

pickup pencircle scaled 1.5pt;
draw a--b--c--a;
pair p[];path l[];

p1:=(n-1)/n*b;p2:=(n-2)/n*b;p3:=(n-3)/n*b;
p4:=p1+1/n*c;p5:=p2+1/n*c;p6:=p3+1/n*c;

p7:=CC-(0.3,0.3)*u;p8:=p7+1/n*b;p9:=p7+1/n*c;p10:=p9+1/n*b;

p11:=1/n*b;p12:=1/n*c;p13:=p12+1/n*b;
p14:=(n-1)/n*c;p15:=(n-2)/n*c;p16:=p14+1/n*b;p17:=p15+1/n*b;

p18:=p5+1/n*c;p19:=p6+1/n*c;

l1:=p1--p4;l2:=p2--p18;l3:=p3--p19+(0.4,0)*u;
l4:=p8-(0.4,0)*u--p10+(0.4,0)*u;l5:=p7-(0.4,0)*u--p9+(0.4,0)*u;
l6:=p4--p6+dir(-120)*0.4u;l7:=p18--p19+dir(-120)*0.4u;
l8:=p8+dir(60)*0.4u--p7+dir(-120)*0.4u;l9:=p10+dir(60)*0.4u--p9+dir(-120)*0.4u;

l10:=p11--p13+(0.4,0)*u;l11:=p17-(0.4,0)*u--p16;
l12:=p13+dir(60)*0.4u--p12;l13:=p17+dir(60)*0.4u--p15;l14:=p16--p14;

pair q[];path m[];

for i=1 upto 19:
  q[i]:=p[i] rotatedaround(CC,240) reflectedabout(b,1/2[a,c]);
  draw q[i] withpen pencircle scaled 2.5bp;
endfor;

for i=1 upto 14:
  m[i]:=l[i]:=l[i] rotatedaround(CC,240) reflectedabout(b,1/2[a,c]);
endfor;

for i=1 upto 9:
  draw m[i] dashed evenly scaled 1;
endfor;

draw subpath(0.2,1) of m13 dashed evenly scaled 1;
draw subpath(0,0.22) of m10 dashed evenly scaled 1;draw subpath(0.8,1) of m10 dashed evenly scaled 1;
draw subpath(0,0.22) of m12 dashed evenly scaled 1;draw subpath(0.8,1) of m12 dashed evenly scaled 1;
draw subpath(0,0.4) of m11 dashed evenly scaled 1;draw subpath(0.8,1) of m11 dashed evenly scaled 1;
draw subpath(0,0.22) of m14 dashed evenly scaled 1;draw subpath(0.8,1) of m14 dashed evenly scaled 1;

label.lft(btex $(1,1)$ etex scaled 0.9,q5+(0.01,0)*u);
label.top(btex $(1,n-1)$ etex scaled 0.9,q13);
label.lft(btex $(1,2)$ etex scaled 0.9,q6+(0.02,0)*u);
label.lft(btex $(2,1)$ etex scaled 0.9,q19+(0.02,0)*u);
label.lft(btex $(r,s)$ etex scaled 0.9,q9+(0.01,0)*u);
label.lft(btex $(n-1,1)$ etex scaled 0.9,q14+(0.26,-0.4)*u);

dotlabel.lft(btex $b$ etex scaled 1,q7);
dotlabel.lft(btex $c$ etex scaled 1,q8);
dotlabel.rt(btex $d$ etex scaled 1,q9);
dotlabel.rt(btex $a$ etex scaled 1,q10);


endfig;

beginfig(11);
label.llft(btex $i$ etex scaled 1.2,a);
label.top(btex $j$ etex scaled 1.2,b);
label.lrt(btex $k$ etex scaled 1.2,c);;

pickup pencircle scaled 1.5pt;
draw a--b--c--a;
pair p[];path l[];

p1:=(n-1)/n*b;p2:=(n-2)/n*b;p3:=(n-3)/n*b;
p4:=p1+1/n*c;p5:=p2+1/n*c;p6:=p3+1/n*c;

p7:=CC-(0.3,0.3)*u;p8:=p7+1/n*b;p9:=p7+1/n*c;p10:=p9+1/n*b;

p11:=1/n*b;p12:=1/n*c;p13:=p12+1/n*b;
p14:=(n-1)/n*c;p15:=(n-2)/n*c;p16:=p14+1/n*b;p17:=p15+1/n*b;

p18:=p5+1/n*c;p19:=p6+1/n*c;

l1:=p1--p4;l2:=p2--p18;l3:=p3--p19+(0.4,0)*u;
l4:=p8-(0.4,0)*u--p10+(0.4,0)*u;l5:=p7-(0.4,0)*u--p9+(0.4,0)*u;
l6:=p4--p6+dir(-120)*0.4u;l7:=p18--p19+dir(-120)*0.4u;
l8:=p8+dir(60)*0.4u--p7+dir(-120)*0.4u;l9:=p10+dir(60)*0.4u--p9+dir(-120)*0.4u;

l10:=p11--p13+(0.4,0)*u;l11:=p17-(0.4,0)*u--p16;
l12:=p13+dir(60)*0.4u--p12;l13:=p17+dir(60)*0.4u--p15;l14:=p16--p14;

pair q[];path m[];

for i=1 upto 19:
  q[i]:=p[i] rotatedaround(CC,120);
  draw q[i] withpen pencircle scaled 2.5bp;
endfor;

for i=1 upto 14:
  m[i]:=l[i]:=l[i] rotatedaround(CC,120);
endfor;

for i=1 upto 9:
  draw m[i] dashed evenly scaled 1;
endfor;

draw m13 dashed evenly scaled 1;
draw m14 dashed evenly scaled 1;
draw m12 dashed evenly scaled 1;
draw subpath(0,0.22) of m10 dashed evenly scaled 1;draw subpath(0.6,1) of m10 dashed evenly scaled 1;
draw subpath(0,0.22) of m11 dashed evenly scaled 1;draw subpath(0.8,1) of m11 dashed evenly scaled 1;

label.llft(btex $(1,1)$ etex scaled 0.9,q5+(0.19,-0.14)*u);
label.llft(btex $(1,n-1)$ etex scaled 0.9,q12+(0.16,-0.14)*u);
label.llft(btex $(1,2)$ etex scaled 0.9,q6+(0.19,-0.14)*u);
label.llft(btex $(2,1)$ etex scaled 0.9,q19+(0.19,-0.14)*u);
label.llft(btex $(r,s)$ etex scaled 0.9,q9+(0.17,-0.14)*u);
label.top(btex $(n-1,1)$ etex scaled 0.9,q17);

dotlabel.llft(btex $b$ etex scaled 1,q7);
dotlabel.llft(btex $c$ etex scaled 1,q8);
dotlabel.urt(btex $d$ etex scaled 1,q9);
dotlabel.urt(btex $a$ etex scaled 1,q10);

endfig;

beginfig(12);

pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;

dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.ulft(btex $3$ etex scaled 1.8,b);
dotlabel.lrt(btex $1$ etex scaled 1.8,c);
dotlabel.urt(btex $2$ etex scaled 1.8,d);

draw 1/3[a,b] withpen pencircle scaled 4bp;
draw 2/3[a,b] withpen pencircle scaled 4bp;
draw 1/3[a,c] withpen pencircle scaled 4bp;
draw 2/3[a,c] withpen pencircle scaled 4bp;
draw 1/3[a,d] withpen pencircle scaled 4bp;
draw 2/3[a,d] withpen pencircle scaled 4bp;
draw 1/3[b,d] withpen pencircle scaled 4bp;
draw 2/3[b,d] withpen pencircle scaled 4bp;
draw 1/3[b,c] withpen pencircle scaled 4bp;
draw 2/3[b,c] withpen pencircle scaled 4bp;
draw 1/3[c,d] withpen pencircle scaled 4bp;
draw 2/3[c,d] withpen pencircle scaled 4bp;

draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;
draw 1/2[2/3[b,c],2/3[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/3[a,b],2/3[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/3[a,d],1/3[c,d]] withpen pencircle scaled 4bp;

ahlength:=10;
singlearrow a--1/2[a,b];singlearrow c--1/2[c,b];
doublearrow a--1/2[a,c];doublearrow a--7/24[a,d];
whitearrow c--1/2[c,d];whitearrow d--1/2[b,d];

label.ulft(btex $a_0$ etex scaled 1.5,1/3[a,b]);
label.ulft(btex $a_1$ etex scaled 1.5,2/3[a,b]);
label.bot(btex $b_0$ etex scaled 1.5,1/3[a,c]);
label.bot(btex $b_1$ etex scaled 1.5,2/3[a,c]);
label.ulft(btex $b_0$ etex scaled 1.5,1/3[a,d]);
label.ulft(btex $b_1$ etex scaled 1.5,2/3[a,d]);
label.urt(btex $a_1$ etex scaled 1.5,1/3[b,c]);
label.urt(btex $a_0$ etex scaled 1.5,2/3[b,c]);
label.top(btex $c_1$ etex scaled 1.5,1/3[b,d]);
label.top(btex $c_0$ etex scaled 1.5,2/3[b,d]);
label.urt(btex $c_0$ etex scaled 1.5,1/3[c,d]+(0.1,0)*u);
label.urt(btex $c_1$ etex scaled 1.5,2/3[c,d]+(0.1,0)*u);
label.urt(btex $x_2$ etex scaled 1.5,1/2[1/3[a,b],1/3[c,b]]);
label.urt(btex $x_0$ etex scaled 1.5,1/2[1/3[c,b],1/3[d,b]]);
label.ulft(btex $x_1$ etex scaled 1.5,1/2[1/3[a,b],1/3[d,b]]);
label.ulft(btex $x_3$ etex scaled 1.5,1/2[1/3[a,d],1/3[c,d]]);

endfig;

beginfig(13);

pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;

dotlabel.llft(btex $1$ etex scaled 1.8,a);
dotlabel.ulft(btex $3$ etex scaled 1.8,b);
dotlabel.lrt(btex $2$ etex scaled 1.8,c);
dotlabel.urt(btex $0$ etex scaled 1.8,d);

draw 1/3[a,b] withpen pencircle scaled 4bp;
draw 2/3[a,b] withpen pencircle scaled 4bp;
draw 1/3[a,c] withpen pencircle scaled 4bp;
draw 2/3[a,c] withpen pencircle scaled 4bp;
draw 1/3[a,d] withpen pencircle scaled 4bp;
draw 2/3[a,d] withpen pencircle scaled 4bp;
draw 1/3[b,d] withpen pencircle scaled 4bp;
draw 2/3[b,d] withpen pencircle scaled 4bp;
draw 1/3[b,c] withpen pencircle scaled 4bp;
draw 2/3[b,c] withpen pencircle scaled 4bp;
draw 1/3[c,d] withpen pencircle scaled 4bp;
draw 2/3[c,d] withpen pencircle scaled 4bp;

draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;
draw 1/2[2/3[b,c],2/3[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/3[a,b],2/3[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/3[a,d],1/3[c,d]] withpen pencircle scaled 4bp;

singlearrow d--1/2[b,d];singlearrow 0.52*d--7/24[a,d];
doublearrow a--1/2[a,c];doublearrow a--1/2[a,b];
whitearrow c--1/2[c,b];whitearrow d--1/2[c,d];


label.ulft(btex $b_0$ etex scaled 1.5,1/3[a,b]);
label.ulft(btex $b_1$ etex scaled 1.5,2/3[a,b]);
label.bot(btex $b_0$ etex scaled 1.5,1/3[a,c]);
label.bot(btex $b_1$ etex scaled 1.5,2/3[a,c]);
label.ulft(btex $a_1$ etex scaled 1.5,1/3[a,d]);
label.ulft(btex $a_0$ etex scaled 1.5,2/3[a,d]);
label.urt(btex $c_1$ etex scaled 1.5,1/3[b,c]);
label.urt(btex $c_0$ etex scaled 1.5,2/3[b,c]);
label.top(btex $a_1$ etex scaled 1.5,1/3[b,d]);
label.top(btex $a_0$ etex scaled 1.5,2/3[b,d]);
label.urt(btex $c_1$ etex scaled 1.5,1/3[c,d]+(0.1,0)*u);
label.urt(btex $c_0$ etex scaled 1.5,2/3[c,d]+(0.1,0)*u);
label.urt(btex $x_3$ etex scaled 1.5,1/2[1/3[a,b],1/3[c,b]]);
label.urt(btex $x_0$ etex scaled 1.5,1/2[1/3[c,b],1/3[d,b]]);
label.ulft(btex $y_2$ etex scaled 1.5,1/2[1/3[a,b],1/3[d,b]]);
label.ulft(btex $y_3$ etex scaled 1.5,1/2[1/3[a,d],1/3[c,d]]);

endfig;

beginfig(14);

pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;

dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.ulft(btex $1$ etex scaled 1.8,b);
dotlabel.lrt(btex $2$ etex scaled 1.8,c);
dotlabel.urt(btex $3$ etex scaled 1.8,d);

draw 1/3[a,b] withpen pencircle scaled 4bp;
draw 2/3[a,b] withpen pencircle scaled 4bp;
draw 1/3[a,c] withpen pencircle scaled 4bp;
draw 2/3[a,c] withpen pencircle scaled 4bp;
draw 1/3[a,d] withpen pencircle scaled 4bp;
draw 2/3[a,d] withpen pencircle scaled 4bp;
draw 1/3[b,d] withpen pencircle scaled 4bp;
draw 2/3[b,d] withpen pencircle scaled 4bp;
draw 1/3[b,c] withpen pencircle scaled 4bp;
draw 2/3[b,c] withpen pencircle scaled 4bp;
draw 1/3[c,d] withpen pencircle scaled 4bp;
draw 2/3[c,d] withpen pencircle scaled 4bp;

draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;
draw 1/2[2/3[b,c],2/3[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/3[a,b],2/3[b,d]] withpen pencircle scaled 4bp;
draw 1/2[1/3[a,d],1/3[c,d]] withpen pencircle scaled 4bp;

singlearrow a--1/2[a,b];singlearrow a--7/24[a,d];
doublearrow a--1/2[a,c];doublearrow d--1/2[b,d];
whitearrow c--1/2[c,b];singlearrow c--1/2[c,d];


label.ulft(btex $a_0$ etex scaled 1.5,1/3[a,b]);
label.ulft(btex $a_1$ etex scaled 1.5,2/3[a,b]);
label.bot(btex $b_0$ etex scaled 1.5,1/3[a,c]);
label.bot(btex $b_1$ etex scaled 1.5,2/3[a,c]);
label.ulft(btex $a_0$ etex scaled 1.5,1/3[a,d]);
label.ulft(btex $a_1$ etex scaled 1.5,2/3[a,d]);
label.urt(btex $c_1$ etex scaled 1.5,1/3[b,c]);
label.urt(btex $c_0$ etex scaled 1.5,2/3[b,c]);
label.top(btex $b_1$ etex scaled 1.5,1/3[b,d]);
label.top(btex $b_0$ etex scaled 1.5,2/3[b,d]);
label.urt(btex $a_0$ etex scaled 1.5,1/3[c,d]+(0.1,0)*u);
label.urt(btex $a_1$ etex scaled 1.5,2/3[c,d]+(0.1,0)*u);
label.urt(btex $x_1$ etex scaled 1.5,1/2[1/3[a,b],1/3[c,b]]);
label.urt(btex $y_3$ etex scaled 1.5,1/2[1/3[c,b],1/3[d,b]]);
label.ulft(btex $y_2$ etex scaled 1.5,1/2[1/3[a,b],1/3[d,b]]);
label.ulft(btex $x_2$ etex scaled 1.5,1/2[1/3[a,d],1/3[c,d]]);

endfig;

beginfig(15);

pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;

p0:=1/5[1/2[c,d],b];p1:=1/4[1/2[a,c],d];
p2:=1/3[1/2[a,d],b]-(0.5,0.2)*u;p3:=1/4[1/2[a,c],b];

draw (p0-0.05*(d-c))--(p0+0.05*(d-c));
draw (p0-0.05*(b-1/2[c,d]))--(p0+0.05*(b-1/2[c,d]));
%draw (p0-0.04*(b-1/2[c,d])) withpen pencircle scaled 3bp;
%draw (p0+0.04*(b-1/2[c,d])) withpen pencircle scaled 3bp;

draw (p1-0.04*c)--(p1+0.04*c);
draw (p1-0.033*(1/2[a,c]-d))--(p1+0.033*(1/2[a,c]-d));
%draw (p1-0.03*(1/2[a,c]-d)) withpen pencircle scaled 3bp;
%draw (p1+0.03*(1/2[a,c]-d)) withpen pencircle scaled 3bp;

draw (p2-0.03*d)--(p2+0.03*d);
%draw (p2-0.1*(b-1/2[a,d]))--(p2+0.1*(b-1/2[a,d]));
draw (p2-0.08*(b-1/2[a,d])) withpen pencircle scaled 3bp;
draw (p2+0.08*(b-1/2[a,d])) withpen pencircle scaled 3bp;

draw (p3-0.04*c)--(p3+0.04*c);
%draw (p3-(0,0.3)*u)--(p3+(0,0.3)*u);
draw (p3-(0,0.22)*u) withpen pencircle scaled 3bp;
draw (p3+(0,0.22)*u) withpen pencircle scaled 3bp;




dotlabel.llft(btex $2$ etex scaled 1.8,a);
dotlabel.ulft(btex $3$ etex scaled 1.8,b);
dotlabel.lrt(btex $1$ etex scaled 1.8,c);
dotlabel.urt(btex $0$ etex scaled 1.8,d);


%draw 1/3[a,b] withpen pencircle scaled 4bp;
%draw 2/3[a,b] withpen pencircle scaled 4bp;
%draw 1/3[a,c] withpen pencircle scaled 4bp;
%draw 2/3[a,c] withpen pencircle scaled 4bp;
%draw 1/3[a,d] withpen pencircle scaled 4bp;
%draw 2/3[a,d] withpen pencircle scaled 4bp;
%draw 1/3[b,d] withpen pencircle scaled 4bp;
%draw 2/3[b,d] withpen pencircle scaled 4bp;
%draw 1/3[b,c] withpen pencircle scaled 4bp;
%draw 2/3[b,c] withpen pencircle scaled 4bp;
%draw 1/3[c,d] withpen pencircle scaled 4bp;
%draw 2/3[c,d] withpen pencircle scaled 4bp;

%draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;
%draw 1/2[2/3[b,c],2/3[b,d]] withpen pencircle scaled 4bp;
%draw 1/2[1/3[a,b],2/3[b,d]] withpen pencircle scaled 4bp;
%draw 1/2[1/3[a,d],1/3[c,d]] withpen pencircle scaled 4bp;

%singlearrow c--1/2[c,b];singlearrow c--1/2[c,a];singlearrow 1/2[a,d]--7/24[a,d];
%doublearrow a--1/2[a,b];doublearrow d--1/2[b,d];doublearrow d--1/2[d,c];

draw 1/2[a,b] withpen pencircle scaled 4bp;
draw 1/2[a,c] withpen pencircle scaled 4bp;
draw 1/2[b,c] withpen pencircle scaled 4bp;
draw 1/2[c,d] withpen pencircle scaled 4bp;
draw 1/2[a,d] withpen pencircle scaled 4bp;
draw 1/2[b,d] withpen pencircle scaled 4bp;

label.ulft(btex $y$ etex scaled 1.7,1/2[a,b]); 
label.rt(btex $y$ etex scaled 1.7,1/2[c,d]);
label.top(btex $y$ etex scaled 1.7,1/2[b,d]);
label.bot(btex $x$ etex scaled 1.7,1/2[a,c]);
label.urt(btex $x$ etex scaled 1.7,1/2[c,b]);
label.lrt(btex $x$ etex scaled 1.7,1/2[a,d]);

singlearrow c--1/3[c,b];singlearrow c--1/3[c,a];singlearrow d--1/3[d,a];
doublearrow a--1/3[a,b];doublearrow d--1/3[d,b];doublearrow d--1/3[d,c];


endfig;

beginfig(16);

pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;

draw (p0-0.05*(d-c))--(p0+0.05*(d-c));
draw (p0-0.05*(b-1/2[c,d]))--(p0+0.05*(b-1/2[c,d]));
%draw (p0-0.04*(b-1/2[c,d])) withpen pencircle scaled 3bp;
%draw (p0+0.04*(b-1/2[c,d])) withpen pencircle scaled 3bp;

draw (p1-0.04*c)--(p1+0.04*c);
%draw (p1-0.033*(1/2[a,c]-d))--(p1+0.033*(1/2[a,c]-d));
draw (p1-0.03*(1/2[a,c]-d)) withpen pencircle scaled 3bp;
draw (p1+0.03*(1/2[a,c]-d)) withpen pencircle scaled 3bp;

draw (p2-0.03*d)--(p2+0.03*d);
draw (p2-0.1*(b-1/2[a,d]))--(p2+0.1*(b-1/2[a,d]));
%draw (p2-0.08*(b-1/2[a,d])) withpen pencircle scaled 3bp;
%draw (p2+0.08*(b-1/2[a,d])) withpen pencircle scaled 3bp;

draw (p3-0.04*c)--(p3+0.04*c);
%draw (p3-(0,0.3)*u)--(p3+(0,0.3)*u);
draw (p3-(0,0.22)*u) withpen pencircle scaled 3bp;
draw (p3+(0,0.22)*u) withpen pencircle scaled 3bp;

dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.ulft(btex $3$ etex scaled 1.8,b);
dotlabel.lrt(btex $1$ etex scaled 1.8,c);
dotlabel.urt(btex $2$ etex scaled 1.8,d);

%draw 1/3[a,b] withpen pencircle scaled 4bp;
%draw 2/3[a,b] withpen pencircle scaled 4bp;
%draw 1/3[a,c] withpen pencircle scaled 4bp;
%draw 2/3[a,c] withpen pencircle scaled 4bp;
%draw 1/3[a,d] withpen pencircle scaled 4bp;
%draw 2/3[a,d] withpen pencircle scaled 4bp;
%draw 1/3[b,d] withpen pencircle scaled 4bp;
%draw 2/3[b,d] withpen pencircle scaled 4bp;
%draw 1/3[b,c] withpen pencircle scaled 4bp;
%draw 2/3[b,c] withpen pencircle scaled 4bp;
%draw 1/3[c,d] withpen pencircle scaled 4bp;
%draw 2/3[c,d] withpen pencircle scaled 4bp;

%draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;
%draw 1/2[2/3[b,c],2/3[b,d]] withpen pencircle scaled 4bp;
%draw 1/2[1/3[a,b],2/3[b,d]] withpen pencircle scaled 4bp;
%draw 1/2[1/3[a,d],1/3[c,d]] withpen pencircle scaled 4bp;

%singlearrow a--1/2[a,b];singlearrow a--1/2[a,c];singlearrow d--1/2[d,b];
%doublearrow a--7/24[a,d];doublearrow c--1/2[b,c];doublearrow c--1/2[c,d];

draw 1/2[a,b] withpen pencircle scaled 4bp;
draw 1/2[a,c] withpen pencircle scaled 4bp;
draw 1/2[b,c] withpen pencircle scaled 4bp;
draw 1/2[c,d] withpen pencircle scaled 4bp;
draw 1/2[a,d] withpen pencircle scaled 4bp;
draw 1/2[b,d] withpen pencircle scaled 4bp;

label.ulft(btex $x$ etex scaled 1.7,1/2[a,b]); 
label.rt(btex $y$ etex scaled 1.7,1/2[c,d]);
label.top(btex $x$ etex scaled 1.7,1/2[b,d]);
label.bot(btex $x$ etex scaled 1.7,1/2[a,c]);
label.urt(btex $y$ etex scaled 1.7,1/2[c,b]);
label.lrt(btex $y$ etex scaled 1.7,1/2[a,d]);

singlearrow a--1/3[a,b];singlearrow a--1/3[a,c];singlearrow d--1/3[d,b];
doublearrow a--1/3[a,d];doublearrow c--1/3[c,b];doublearrow c--1/3[c,d];

endfig;

beginfig(17);

pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;

p0:=1/5[1/2[c,d],b];p1:=1/4[1/2[a,c],d];
p2:=1/3[1/2[a,d],b]-(0.5,0.2)*u;p3:=1/4[1/2[a,c],b];

draw (p0-0.05*(d-c))--(p0+0.05*(d-c));
%draw (p0-0.05*(b-1/2[c,d]))--(p0+0.05*(b-1/2[c,d]));
draw (p0-0.04*(b-1/2[c,d])) withpen pencircle scaled 3bp;
draw (p0+0.04*(b-1/2[c,d])) withpen pencircle scaled 3bp;

draw (p1-0.04*c)--(p1+0.04*c);
draw (p1-0.033*(1/2[a,c]-d))--(p1+0.033*(1/2[a,c]-d));
%draw (p1-0.03*(1/2[a,c]-d)) withpen pencircle scaled 3bp;
%draw (p1+0.03*(1/2[a,c]-d)) withpen pencircle scaled 3bp;

draw (p2-0.03*d)--(p2+0.03*d);
draw (p2-0.1*(b-1/2[a,d]))--(p2+0.1*(b-1/2[a,d]));
%draw (p2-0.08*(b-1/2[a,d])) withpen pencircle scaled 3bp;
%draw (p2+0.08*(b-1/2[a,d])) withpen pencircle scaled 3bp;

draw (p3-0.04*c)--(p3+0.04*c);
%draw (p3-(0,0.3)*u)--(p3+(0,0.3)*u);
draw (p3-(0,0.22)*u) withpen pencircle scaled 3bp;
draw (p3+(0,0.22)*u) withpen pencircle scaled 3bp;

label.ulft(btex $0$ etex scaled 1.8,a+(0,0.1)*u);
label.llft(btex $1$ etex scaled 1.8,b-(0.3,0.1)*u);
label.urt(btex $2$ etex scaled 1.8,c+(0.2,0.1)*u);
label.lrt(btex $3$ etex scaled 1.8,d-(0,0.1)*u);

dotlabel.llft(btex $\alpha^{-1}N$ etex scaled 1.8,a);
dotlabel.ulft(btex $N$ etex scaled 1.8,b);
dotlabel.lrt(btex $\alpha N$ etex scaled 1.8,c);
dotlabel.urt(btex $\alpha^2N$ etex scaled 1.8,d);


%draw 1/3[a,b] withpen pencircle scaled 4bp;
%draw 2/3[a,b] withpen pencircle scaled 4bp;
%draw 1/3[a,c] withpen pencircle scaled 4bp;
%draw 2/3[a,c] withpen pencircle scaled 4bp;
%draw 1/3[a,d] withpen pencircle scaled 4bp;
%draw 2/3[a,d] withpen pencircle scaled 4bp;
%draw 1/3[b,d] withpen pencircle scaled 4bp;
%draw 2/3[b,d] withpen pencircle scaled 4bp;
%draw 1/3[b,c] withpen pencircle scaled 4bp;
%draw 2/3[b,c] withpen pencircle scaled 4bp;
%draw 1/3[c,d] withpen pencircle scaled 4bp;
%draw 2/3[c,d] withpen pencircle scaled 4bp;

%draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;
%draw 1/2[2/3[b,c],2/3[b,d]] withpen pencircle scaled 4bp;
%draw 1/2[1/3[a,b],2/3[b,d]] withpen pencircle scaled 4bp;
%draw 1/2[1/3[a,d],1/3[c,d]] withpen pencircle scaled 4bp;

%singlearrow a--1/2[a,b];singlearrow b--1/2[b,c];singlearrow c--1/2[c,d];
%doublearrow a--7/24[a,d];whitearrow a--1/2[a,c];whitearrow b--1/2[b,d];

draw 1/2[a,b] withpen pencircle scaled 4bp;
draw 1/2[a,c] withpen pencircle scaled 4bp;
draw 1/2[b,c] withpen pencircle scaled 4bp;
draw 1/2[c,d] withpen pencircle scaled 4bp;
draw 1/2[a,d] withpen pencircle scaled 4bp;
draw 1/2[b,d] withpen pencircle scaled 4bp;

label.ulft(btex $x$ etex scaled 1.7,1/2[a,b]); 
label.rt(btex $x$ etex scaled 1.7,1/2[c,d]);
label.top(btex $y$ etex scaled 1.7,1/2[b,d]);
label.bot(btex $y$ etex scaled 1.7,1/2[a,c]);
label.urt(btex $x$ etex scaled 1.7,1/2[c,b]);
label.lrt(btex $z$ etex scaled 1.7,1/2[a,d]);

singlearrow a--1/3[a,b];singlearrow b--1/3[b,c];singlearrow c--1/3[c,d];
whitearrow a--1/3[a,d];doublearrow a--1/3[a,c];doublearrow b--1/3[b,d];

endfig;

beginfig(18);

pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;

p0:=1/5[1/2[c,d],b];p1:=1/4[1/2[a,c],d];
p2:=1/3[1/2[a,d],b]-(0.5,0.2)*u;p3:=1/4[1/2[a,c],b];

draw (p0-0.05*(d-c))--(p0+0.05*(d-c));
draw (p0-0.05*(b-1/2[c,d]))--(p0+0.05*(b-1/2[c,d]));
%draw (p0-0.04*(b-1/2[c,d])) withpen pencircle scaled 3bp;
%draw (p0+0.04*(b-1/2[c,d])) withpen pencircle scaled 3bp;

draw (p1-0.04*c)--(p1+0.04*c);
draw (p1-0.033*(1/2[a,c]-d))--(p1+0.033*(1/2[a,c]-d));
%draw (p1-0.03*(1/2[a,c]-d)) withpen pencircle scaled 3bp;
%draw (p1+0.03*(1/2[a,c]-d)) withpen pencircle scaled 3bp;

draw (p2-0.03*d)--(p2+0.03*d);
draw (p2-0.1*(b-1/2[a,d]))--(p2+0.1*(b-1/2[a,d]));
%draw (p2-0.08*(b-1/2[a,d])) withpen pencircle scaled 3bp;
%draw (p2+0.08*(b-1/2[a,d])) withpen pencircle scaled 3bp;

draw (p3-0.04*c)--(p3+0.04*c);
draw (p3-(0,0.3)*u)--(p3+(0,0.3)*u);
%draw (p3-(0,0.22)*u) withpen pencircle scaled 3bp;
%draw (p3+(0,0.22)*u) withpen pencircle scaled 3bp;

label.ulft(btex $0$ etex scaled 1.8,a+(0,0.1)*u);
label.llft(btex $3$ etex scaled 1.8,b-(0.3,0.1)*u);
label.urt(btex $2$ etex scaled 1.8,c+(0.2,0.1)*u);
label.lrt(btex $1$ etex scaled 1.8,d-(0,0.1)*u);

dotlabel.llft(btex $\alpha^{-1}N$ etex scaled 1.8,a);
dotlabel.ulft(btex $N$ etex scaled 1.8,b);
dotlabel.lrt(btex $\alpha N$ etex scaled 1.8,c);
dotlabel.urt(btex $\alpha^2N$ etex scaled 1.8,d);

%draw 1/3[a,b] withpen pencircle scaled 4bp;
%draw 2/3[a,b] withpen pencircle scaled 4bp;
%draw 1/3[a,c] withpen pencircle scaled 4bp;
%draw 2/3[a,c] withpen pencircle scaled 4bp;
%draw 1/3[a,d] withpen pencircle scaled 4bp;
%draw 2/3[a,d] withpen pencircle scaled 4bp;
%draw 1/3[b,d] withpen pencircle scaled 4bp;
%draw 2/3[b,d] withpen pencircle scaled 4bp;
%draw 1/3[b,c] withpen pencircle scaled 4bp;
%draw 2/3[b,c] withpen pencircle scaled 4bp;
%draw 1/3[c,d] withpen pencircle scaled 4bp;
%draw 2/3[c,d] withpen pencircle scaled 4bp;

%draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;
%draw 1/2[2/3[b,c],2/3[b,d]] withpen pencircle scaled 4bp;
%draw 1/2[1/3[a,b],2/3[b,d]] withpen pencircle scaled 4bp;
%draw 1/2[1/3[a,d],1/3[c,d]] withpen pencircle scaled 4bp;

%singlearrow a--7/24[a,d];singlearrow c--1/2[c,b];singlearrow d--1/2[c,d];
%doublearrow a--1/2[a,b];
%whitearrow a--1/2[a,c] withpen pencircle scaled 1;whitearrow d--1/2[d,b] withpen pencircle scaled 1;

draw 1/2[a,b] withpen pencircle scaled 4bp;
draw 1/2[a,c] withpen pencircle scaled 4bp;
draw 1/2[b,c] withpen pencircle scaled 4bp;
draw 1/2[c,d] withpen pencircle scaled 4bp;
draw 1/2[a,d] withpen pencircle scaled 4bp;
draw 1/2[b,d] withpen pencircle scaled 4bp;

label.ulft(btex $z$ etex scaled 1.7,1/2[a,b]); 
label.rt(btex $x$ etex scaled 1.7,1/2[c,d]);
label.top(btex $y$ etex scaled 1.7,1/2[b,d]);
label.bot(btex $y$ etex scaled 1.7,1/2[a,c]);
label.urt(btex $x$ etex scaled 1.7,1/2[c,b]);
label.lrt(btex $x$ etex scaled 1.7,1/2[a,d]);

singlearrow a--1/3[a,d];singlearrow c--1/3[c,b];singlearrow d--1/3[d,c];
whitearrow a--1/3[a,b];doublearrow a--1/3[a,c];doublearrow d--1/3[d,b];

endfig;

beginfig(19);
pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw a--c;

dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.top(btex $1$ etex scaled 1.8,b);
dotlabel.lrt(btex $2$ etex scaled 1.8,c);


draw 1/3[a,b] withpen pencircle scaled 4bp;
draw 2/3[a,b] withpen pencircle scaled 4bp;
draw 1/3[a,c] withpen pencircle scaled 4bp;
draw 2/3[a,c] withpen pencircle scaled 4bp;
draw 1/3[b,c] withpen pencircle scaled 4bp;
draw 2/3[b,c] withpen pencircle scaled 4bp;

draw 1/2[1/3[a,b],1/3[c,b]] withpen pencircle scaled 4bp;

label.ulft(btex $a$ etex scaled 1.5,2/3[a,b]);
label.urt(btex $b$ etex scaled 1.5,2/3[c,b]);
label.ulft(btex $c$ etex scaled 1.5,1/3[a,b]);
label.top(btex $d$ etex scaled 1.5,1/2[1/3[a,b],1/3[c,b]]);
label.urt(btex $e$ etex scaled 1.5,2/3[b,c]);
label.top(btex $f$ etex scaled 1.5,1/3[a,c]);
label.top(btex $g$ etex scaled 1.5,2/3[a,c]);

endfig;

beginfig(20);
pickup pencircle scaled 1.5pt;

dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.top(btex $1$ etex scaled 1.8,b);
dotlabel.lrt(btex $2$ etex scaled 1.8,c);

draw 1/4[a,b]--3/4[a,b];draw 3/4[a,b]--1/4[b,c];draw 1/4[b,c]--3/4[b,c];
draw 1/4[a,b]--1/4[a,c];draw 1/4[a,c]--3/4[a,c];draw 3/4[a,c]--1/4[c,b];

draw a--1/4[a,b] dashed evenly scaled 1;
draw a--1/4[a,c] dashed evenly scaled 1;
draw b--1/4[b,a] dashed evenly scaled 1;
draw b--1/4[b,c] dashed evenly scaled 1;
draw c--1/4[c,a] dashed evenly scaled 1;
draw c--1/4[c,b] dashed evenly scaled 1;

singlearrow 1/4[a,b]--1/2[a,b];
singlearrow 1/4[b,c]--1/2[b,c];
singlearrow 1/4[a,c]--1/2[a,c];

singlearrow 1/4[a,b]--1/2[1/4[a,b],1/4[a,c]];
singlearrow 1/4[b,a]--1/2[1/4[b,a],1/4[b,c]];
singlearrow 1/4[c,a]--1/2[1/4[c,a],1/4[c,b]];

label.ulft(btex $q_{01}$ etex scaled 1.5,1/2[a,b]);
label.urt(btex $q_{12}$ etex scaled 1.5,1/2[b,c]);
label.top(btex $q_{02}$ etex scaled 1.5,1/2[a,c]);

label.urt(btex $\alpha^0_{12}$ etex scaled 1.5,1/2[1/4[a,b],1/4[a,c]]);
label.ulft(btex $\alpha^0_{12}$ etex scaled 1.5,1/2[1/4[c,a],1/4[c,b]]);
label.bot(btex $\alpha^1_{02}$ etex scaled 1.5,1/2[1/4[b,a],1/4[b,c]]);

endfig;


beginfig(21);
%pickup pencircle scaled 1.5pt;
pair P[]; pair Q[];
P1:=(2,0)*u;P2:=(0,2)*u;P3:=(-2,0)*u;P4:=(0,-2)*u;
Q1:=dir(60)*2*u;Q2:=dir(160)*2*u;Q3:=dir(-150)*2*u;Q4:=dir(-10)*2*u;
draw P1..P2..P3..P4..P1 dashed evenly;
draw Q1--Q2;draw Q3--Q4;draw Q1--Q3;draw Q1--Q4;draw Q2--Q3;draw Q2--Q4;
label.rt(btex $c$ etex,1/2[Q2,Q3]);
label.top(btex $a$ etex,1/2[Q1,Q2]);
label.bot(btex $b$ etex,1/2[Q3,Q4]);
label.lft(btex $d$ etex,1/2[Q1,Q4]);
label.rt(btex $e$ etex,1/4[Q3,Q1]);
label.top(btex $f$ etex,1/2[Q2,Q4]);

endfig;

beginfig(22);
pickup pencircle scaled 1.5pt;
draw a--b; draw b--c;draw c--d;
draw b--d; draw a--c;
draw a--0.52*d; draw 0.58*d--d;

dotlabel.llft(btex $0$ etex scaled 1.8,a);
dotlabel.ulft(btex $1$ etex scaled 1.8,b);
dotlabel.lrt(btex $2$ etex scaled 1.8,c);
dotlabel.urt(btex $3$ etex scaled 1.8,d);

label.lft(btex $z$ etex scaled 1.8,1/2[a,b]);
label.rt(btex $z$ etex scaled 1.8,1/2[c,d]);
label.urt(btex $z^\prime$ etex scaled 1.8,1/2[b,c]);
label.rt(btex $z^\prime$ etex scaled 1.8,1/3[a,d]);
label.top(btex $z^{\prime\prime}$ etex scaled 1.8,1/2[b,d]);
label.bot(btex $z^{\prime\prime}$ etex scaled 1.8,1/2[a,c]);

endfig;

end;




